Gyojas $W$-Graph-Algebra und zellul\"are Struktur von Iwahori-Hecke-Algebren

On overview of Coxeter groups $W$, their Iwahori-Hecke algebras $H$, Lusztig's asymptotic algebras $J$, cellular algebras in general and cellularity of $H$ in particular, as well as an introduction to Gyoja's $W$-graph algebra and the $W$-graph decomposition conjecture.

==> aussortiertes.tex <==
	\item	Auf Pfad-Algebren ist die natürliche Graduierung durch die Pfad-Länge gegeben. Diese induziert auf $\Omega$ zwar keine Graduierung aber eine Filtrierung:
\[F^{\leq k}\Omega = \operatorname{span}\Set{E_I, X_{I_0 I_1} X_{I_1 I_2} \ldots X_{I_{m-1} I_m} | m\leq k, I_j\subseteq S}\]
Es nun naheliegend, die assoziierte graduierte Algebra $\operatorname{gr}\Omega=\bigoplus_{k\in\IN} F^{\leq k}\Omega/F^{\leq k-1}\Omega$ zu untersuchen. Eine interessante Beobachtung ist beispielsweise, dass $s\mapsto x_s$ einen Homomorphismus von der Nil-Hecke-Algebra nach $\operatorname{gr}\Omega$ definiert.
	\index{terms}{Graduierung}\index{terms}{Filtrierung}

















Es stellt sich heraus, dass $\OmegaGy$ nicht nur Quotient der Pfadalgebra $\Xi=\IZ\mathcal{Q}$ ist, denn $\IZ\mathcal{Q}\to\OmegaGy$ faktorisiert durch eine andere Pfadalgebra mit einem deutlich einfacheren Köcher $\mathcal{Q}_{W,L}$.

Das folgende Lemma ist im Einparameterfall bereits in den Relationen aus Satz \ref{wgraph_alg:relations} enthalten, gilt jedoch auch im Multiparameterfall. Für den Einparameterfall wird hier jedoch ein unabhängiger Beweis dieser einen Relation gegeben, der sich bereits in \citep[2.5]{Gyoja} findet und hier auf den Multiparameterfall ausgeweitet wird.
\begin{lemma}[$X_{IJ}^s$ ist von $s$ unabhängig]\label{wgraph_alg:X_IJ_independent}
\index{symbols}{$X_{IJ}^s$}\index{symbols}{$X_{IJ}$}
Seien $I,J\subseteq S$ und $s,t\in I\setminus J$ mit $\ord(st)<\infty$. Dann gelten folgende Relationen in $\OmegaGy$:
\begin{enumerate}
	\item Ist $L(s)=L(t)>0$, so gilt $X_{IJ}^s = X_{IJ}^t$.
	\item Ist $L(s)>L(t)>0$, so gilt $X_{IJ}^t = 0$.
	\item Wenn $\Set{L(s),L(t)}\subseteq\Gamma$ linear unabhängig über $\IZ$ ist, so ist $X_{IJ}^s = X_{IJ}^t = 0$.
\end{enumerate}
\end{lemma}
\begin{proof}
Wir rechnen in $\IZ[\Gamma] \otimes_\IZ \OmegaGy$.

\medskip
Schritt 1: Rechnen.

Zunächst einmal gilt:
\begin{align*}
	e_s T_s &= -v_s^{-1} e_s^2 + v_s e_s(1-e_s) + e_s x_s \\
	&= -v_s^{-1} e_s + x_s
\end{align*}
Wir berechnen für $m\in\IN_{\geq 2}$ den Ausdruck
\[e_t e_s\underbrace{v_s^{-1} T_s \cdot v_t^{-1} T_t \ldots}_{m}\]
wie folgt
\begin{align*}
	\ldots &= e_t\cdot (e_s v_s^{-1} T_s) \cdot \underbrace{v_t^{-1} T_t v_s^{-1} T_s \ldots }_{m-1} \\
	&= e_t \cdot (-v_s^{-2} e_s + v_s^{-1} x_s) \underbrace{v_t^{-1} T_t v_s^{-1} T_s \ldots}_{m-1} \\
	&= v_s^{-1} e_t x_s \underbrace{(1-e_t)(1-e_s)\ldots}_{m-1} + \text{Terme mit echt kleinerem Exponenten} \\
	&= v_s^{-1} e_t x_s (1-e_t)^a (1-e_s)^b + \text{Terme mit echt kleinerem Exponenten},
\end{align*}
wobei $a,b\in\IN$ mit $a\geq 1$. Nun gilt für alle $b\in\IN$ jedoch $x_s(1-e_s)^b = x_s$, sodass sich der Term zu
\begin{align*}
	\ldots &= v_s^{-1} e_t x_s (1-e_t) + \text{Terme mit echt kleinerem Exponenten}
\end{align*}
vereinfacht. Wenn wir nun ganz konkret $m=m_{st}$ wählen, gilt $\underbrace{T_s T_t \ldots}_{m} = \underbrace{T_t T_s\ldots}_{m}$ nach Definition. Die Idempotente $e_s$ und $e_t$ kommutieren sowieso, d.\,h. für $L(s)=L(t)$ bleibt der Ausdruck, den wir berechnet haben, unverändert, wenn wir $s$ und $t$ vertauschen. Wir erhalten daher die Aussage
\[e_t x_s (1-e_t) = e_s x_t (1-e_s).\]

Nun schauen wir genauer hin: Der erste Ausdruck hatte seinen höchsten Term im Grad $-L(s)$ und der zweite im Grad $-L(t)$. Wenn nun $L(s)>L(t)$ ist, ist erstens $m_{st}$ gerade (was bedeutet, dass wieder beide Terme übereinstimmen, weil die $v_s$- und $v_t$-Potenzen in beiden dieselben sind) und zweitens $\Gamma_{\leq -L(s)} \subseteq \Gamma_{\leq-L(t)}$. Somit muss der Summand $v_t^{-1} e_s x_t (1-e_s)$ des zweiten Terms verschwinden. Wir erhalten also $e_s x_t (1-e_s) = 0$ in diesem Fall.

Für $s,t\in I\setminus J$ gilt aufgrund der Kommutativität der $e_s$ und der Definition der $E_I$
\[E_I e_s = E_I = E_I e_t\]
sowie
\[(1-e_s)E_J = E_J = (1-e_t) E_J.\]
Daraus folgt
\begin{align*}
	X_{IJ}^t &= E_I x_t E_J \\
	&= E_I e_s x_t (1-e_s) E_J \\
	&= E_I e_t x_s (1-e_t) E_J \\
	&= E_I x_s E_J \\
	&= X_{IJ}^s
\end{align*}
im ersten Fall bzw. im zweiten Fall dann
\begin{align*}
	X_{IJ}^t &= E_I x_t E_J \\
	&= E_I e_s x_t (1-e_s) E_J \\
	&= 0,
\end{align*}
wie gewünscht.

Die dritte Aussage folgt aus der zweiten, wenn man festhält, dass die Ordnung von $\Gamma$ in die Definition von $\OmegaGy(W,S,L)$ überhaupt nicht einging. Die können wir also variieren, ohne Relationen zu verändern. Sind $L(s)$ und $L(t)$ linear unabhängig, dann können wir insbesondere eine Ordnung finden, in der $L(s)>L(t)$ ist, und eine, in der $L(s)<L(t)$ ist. Aus b. folgt dann die Behauptung.
\end{proof}

%\begin{remark}
	%\item Man kann eine Variante dieses Lemmas für $\Omega$ formulieren. Bezeichne mit $\widetilde{\Xi}$ den von $\Set{e_s, x_s | s\in S}$ erzeugten Unterring von $\Omega$. Dann zeigt der gleiche Beweis $L(s)=L(t)>0\implies X_{IJ}^s-X_{IJ}^t \in\IZ[\Gamma_{<0}]\widetilde{\Xi}$, $L(s)>L(t)>0 \implies X_{IJ}^t \in\IZ[\Gamma_{<0}]\widetilde{\Xi}$ sowie $\Set{L(s),L(t)}$ l.u. $\implies X_{IJ}^s, X_{IJ}^t\in\IZ[\Gamma_{<0}]\widetilde{\Xi}$. Ein unmittelbar nützliche Anwendung hiervon ist mir jedoch nicht ersichtlich.
%\end{remark}

\begin{lemma}["`Compatibility rule"', vgl. {\citep[Prop.\,4.1]{Stembridge2008admissble}}]\label{wgraph_alg:comp_rule}
\index{terms}{Kompatibilitätsregel}
Für alle $I,J\subseteq S$ und $s\in I\setminus J$ gilt: Ist $X_{IJ}^s\neq 0$ in $\OmegaGy$, dann gilt für $t\in J\setminus I$ stets $st\neq ts$ oder $L(t)=0$.
\end{lemma}
\begin{proof}
Angenommen, es gibt $t\in J\setminus I$ mit $st=ts$ und $L(t)>0$. Dann betrachten wir $\Delta_2(\iota(T_s),\iota(T_t)) = [\iota(T_s),\iota(T_t)]$ in $\IZ[\Gamma]\Xi$:
\begin{align*}
	\iota(T_s) \iota(T_t) &= (-v_s^{-1} e_s + v_s (1-e_s) + x_s)(-v_t^{-1} e_t + v_t(1-e_t) + x_t) \\
	&= +v_s^{-1} v_t^{-1} e_s e_t \\
	&\phantom{\text{= }} - v_s^{-1} e_s x_t - v_t^{-1} x_s e_t \\
	&\phantom{\text{= }} - v_s^{-1} v_t e_s(1-e_t) - v_s v_t^{-1} (1-e_s) e_t + x_s x_t \\
	&\phantom{\text{= }} + v_s (1-e_s) x_t + v_t x_s(1-e_t) \\
	&\phantom{\text{= }} + v_s v_t e_s e_t \\
\implies \left[\iota(T_s),\iota(T_t)\right] &= -(v_s^{-1}+v_s)[e_s, x_t] + (v_t^{-1}+v_t)[e_t, x_s] + [x_s, x_t]
\end{align*}

Wir multiplizieren den Term nun von links mit $E_I$ und von rechts mit $E_J$. Unter Beachtung von $E_I e_s = E_I$, $E_J e_s = 0$, $E_I e_t = 0$, $E_J e_t = E_J$, erhalten wir:
\begin{align*}
	E_I [\iota(T_s),\iota(T_t)] E_J &= -(v_s^{-1}+v_s) ( \underbrace{E_I e_s x_t E_J}_{=X_{IJ}^t=0} - \underbrace{E_I x_t e_s E_J}_{=0}) \\
	&\phantom{\text{= }} +(v_t^{-1}+v_t) ( \underbrace{E_I e_t x_s E_J}_{=0} - \underbrace{E_I x_s e_t E_J}_{=X_{IJ}^s}) \\
	&\phantom{\text{= }} + \sum_{\substack{K\subseteq S \\ s\in I\setminus K, t\in K\setminus J}} X_{IK}^s X_{KJ}^t
\end{align*}
Da $L(t)>0$ ist, folgt durch Koeffizientenvergleich, dass $X_{IJ}^s = 0$ eine der Relationen in $\OmegaGy$ ist.
\end{proof}

\begin{remark}
\begin{itemize}
	\item Im Einparameterfall ist das die Aussage
	\[X_{IJ}\neq 0 \implies \text{Für alle } s\in I\setminus J, t\in J\setminus I \text{ gilt } st\neq ts.\]
	Dies wird bei Stembridge als "`Compatibility rule"' bezeichnet. Obiges Lemma ist die Verallgemeinerung auf den Multiparameterfall.
	\item Die Aussage ist natürlich trivialerweise wahr, wenn $J\setminus I=\emptyset$ ist. Sie liefert also nur ein Kriterium für die Kanten $J\to I$ im Köcher, die nicht von einer Inklusion herkommen.
	\item Im Einparameterfall folgt insbesondere, dass für transversale Kanten $J \to I$ die Teilmenge $I \Delta J\subseteq S$ des Dynkin-Diagramms einen vollständigen bipartiten Graphen definiert mit $I\setminus J$ und $J\setminus I$ als den zwei Teilen der Bipartition. Unter den endlichen Coxeter-Gruppen sind nur $I_2(m)$, $A_3$, $B_3$, $H_3$ und $D_4$ von dieser Gestalt. Insbesondere folgt $\abs{I \Delta J}\leq 4$.
	\item Auch dieses Lemma folgt im Einparameterfall direkt aus den Relationen aus dem letzten Abschnitt, nämlich aus der Relation $\alpha$: Für $\ord(st)=2$ ist das wegen $\tau_{2-1}(T)=T$ nämlich einfach die Relation $X_{IJ}^s=0$.
\end{itemize}
\end{remark}













\begin{theorem}\label{gyoja:proof_B3}
\index{symbols}{$B_n$}
Gyojas Vermutung ist korrekt für $W=B_3$.
\end{theorem}
\begin{proof}
$B_3$ hat 10 Charaktere. Sie werden durch die $W$-Graphen in Tabelle \ref{tab:w_graphs_B3} realisiert. (Die Kantengewichte sind der Einfachheit halber nur für den Einparameterfall angegeben.)

\begin{table}[hbp]
\begin{tabular}{lcl}
 & Grad & $W$-Graph \\
\hline
$\chi_1=1$               & 1 &
	\begin{tikzpicture} \node[Vertex] at (0,0) {$\emptyset$}; \end{tikzpicture} \\
$\chi_2=\sgn$            & 1 & 
	\begin{tikzpicture} \node[Vertex] at (0,0) {$012$}; \end{tikzpicture} \\
$\chi_3$                 & 1 & 
	\begin{tikzpicture} \node[Vertex] at (0,0) {$0$}; \end{tikzpicture} \\
$\chi_4$                 & 1 & 
	\begin{tikzpicture} \node[Vertex] at (0,0) {$12$}; \end{tikzpicture} \\
$\chi_5$                 & 2 & 
	\begin{tikzpicture}
		\node[Vertex] (E_1) at (0.0,0) {$1$};
		\node[Vertex] (E_2) at (1.5,0) {$2$};
		\path[EdgeT] (E_1) edge node[above]{$1$} (E_2);
	\end{tikzpicture} \\
$\chi_6=\sgn\chi_5$      & 2 & 
	\begin{tikzpicture}
		\node[Vertex] (E_02) at (0.0,0) {$02$};
		\node[Vertex] (E_01) at (1.5,0) {$01$};
		\path[EdgeT] (E_1) edge node[above]{$-1$} (E_2);
	\end{tikzpicture} \\
$\chi_7$                 & 3 & 
	\begin{tikzpicture}
		\node[Vertex] (E_0) at (0.0,0) {$0$};
		\node[Vertex] (E_1) at (1.5,0) {$1$};
		\node[Vertex] (E_2) at (3.0,0) {$2$};
		\path[EdgeT]
			(E_1) edge node[above]{$1$} (E_2);
		\path[EdgeTdir]
			(E_0) edge[bend left=15] node[above]{$2$} (E_1)
			(E_1) edge[bend left=15] node[below]{$1$} (E_0);
	\end{tikzpicture} \\
$\chi_8=\sgn\chi_7$    & 3 & 
	\begin{tikzpicture}
		\node[Vertex] (E_12) at (0.0,0) {$02$};
		\node[Vertex] (E_02) at (1.5,0) {$01$};
		\node[Vertex] (E_01) at (3.0,0) {$12$};
		\path[EdgeT]
			(E_02) edge node[above]{$-1$} (E_01);
		\path[EdgeTdir]
			(E_12) edge[bend left=15] node[above]{$-2$} (E_02)
			(E_02) edge[bend left=15] node[below]{$-1$} (E_12);
	\end{tikzpicture} \\
$\chi_9=\chi_3\chi_7$    & 3 & 
	\begin{tikzpicture}
		\node[Vertex] (E_0)  at (0.0,0) {$0$};
		\node[Vertex] (E_1)  at (1.5,0) {$1$};
		\node[Vertex] (E_02) at (3.0,0) {$02$};
		\path[EdgeT]
			(E_1) edge node[above]{$-1$} (E_0) edge node[above]{$1$} (E_02);
	\end{tikzpicture} \\
$\chi_{10}=\chi_4\chi_7$ & 3 & 
	\begin{tikzpicture}
		\node[Vertex] (E_12) at (0.0,0) {$12$};
		\node[Vertex] (E_02) at (1.5,0) {$02$};
		\node[Vertex] (E_1)  at (3.0,0) {$1$};
		\path[EdgeT]
			(E_02) edge node[above]{$1$} (E_12) edge node[above]{$-1$} (E_1);
	\end{tikzpicture}
\end{tabular}
\caption{$W$-Graphen für $B_3$}
\label{tab:w_graphs_B3}
\end{table}

Schritt 1: $\chi_1$ bis $\chi_4$ sind linear, für die gilt $(\Pi_\lambda)$ bereits. Ebenso gilt dies für die Spiegelungsdarstellung $\chi_7$ und deren Dual $\chi_8$.

\bigskip
Schritt 2: Betrachten wir als ersten offenen Fall die zweidimensionalen Darstellungen.

Wir beweisen $(\Pi_5)$. Seien dafür $X,Y,\alpha$ wie in der Definition. Da in $Y$ nur die $I$-Invarianten $\Set{1}$ und $\Set{2}$ vorkommen, gilt $\alpha(E_I X)=0=E_I Y$ für alle $I\subseteq S$, die keine Teilmenge von $\Set{1}$ oder $\Set{2}$ sind. Für $I=\Set{1}$ und $I=\Set{2}$ gilt ebenfalls $\alpha(E_I X)\subseteq E_I Y$ aufgrund von Lemma \ref{matrices:blocks1}. Damit bleibt nur noch $I=\emptyset$ übrig. Da jedoch weder $X$ noch $Y$ der triviale Modul sind, ist $E_\emptyset X=0$ und $E_\emptyset Y=0$. Das zeigt die $\Omega$-Linearität von $\alpha$. Daher gilt $(\Pi_5)$.

Wir beweisen dual $(\Pi^6)$. Seien dafür $X,Y,\beta$ wie in der Definition. Da in $Y$ nur die $I$-Invarianten $\Set{02}$ und $\Set{01}$ vorkommen, gilt $\beta(E_I Y) = 0 \subseteq E_I X$ für alle $I$, die keine Obermenge von $\Set{02}$ oder $\Set{01}$ sind. Für $I=\Set{012}$ gilt $E_I X=0$, da ansonsten $\text{Res}_H^\Omega(X)$ die Signumsdarstellung als Komponente enthielt, also, da wir $(\Pi^\text{sgn})$ schon bewiesen haben, gleich der Signumsdarstellung sein müsste entgegen der Annahme. Also ist $E_I X = 0$, wie behauptet. Aus Lemma \ref{matrices:blocks1} folgt nun auch $\beta(E_I Y)\subseteq E_I X$ für $I=\Set{01}$ und $I=\Set{02}$. Somit ist $(\Pi^6)$ bewiesen.

\bigskip
Schritt 3: Wir beweisen $(\Pi_9)$. Seien dafür $X,Y,\alpha$ wie in der Definition.

Da wir schon wissen, dass $(\Pi_\lambda)$ für $\lambda\neq 9,10$ gilt, wissen wir, dass die einzigen einfachen $H$-Untermoduln von $X$ vom Isomorphietyp $\chi_9$ und/oder $\chi_{10}$ sind. Insbesondere können die in $X$ vorkommenden $I$-Invarianten höchstens $\Set{0}, \Set{1}, \Set{12}, \Set{02}$ sein.

$Y$ ist vom Isomorphietyp $\chi_9$, hat also die Invarianten $\Set{0}, \Set{1}, \Set{02}$. Da für $I=\emptyset, \Set{2}, \Set{01}, \Set{012}$ bereits $E_I X=0$ gilt, wissen wir, dass $\alpha(E_I X)\subseteq E_I Y$ für diese $I$ erfüllt ist. Aus \ref{matrices:blocks1} folgt dieselbe Inklusion für $I=\Set{1}, \Set{02}, \Set{12}$. Es bleibt also nur noch $I=\Set{0}$ übrig. Hier sagt das Lemma \ref{matrices:blocks1} nur $\alpha(E_{\Set{0}} X)\subseteq E_{\Set{0}} Y + E_{\Set{02}} Y$ voraus.

Aufgrund der Struktur der beiden $W$-Graphen $\chi_9$ und $\chi_{10}$ wissen wir aber mehr, nämlich dass $E_{\Set{0}} X = \operatorname{Eig}_{-v_0^{-1}}(T_0;X) \cap \operatorname{Eig}_{v_2}(T_2;X)$ und daher $\alpha(E_0 X) \subseteq \operatorname{Eig}_{-v_0^{-1}}(T_0;X) \cap \operatorname{Eig}_{v_2}(T_2;X) = E_{\Set{0}} Y$ ist.

\bigskip
Schritt 4: Wir beweisen $(\Pi_{10})$. Seien dafür $X,Y,\alpha$ wie in der Definition.

Da wir schon wissen, dass $(\Pi_\lambda)$ für $\lambda\neq 10$ gilt, wissen wir, dass die einzigen einfachen $H$-Untermoduln von $X$ vom Isomorphietyp $\chi_{10}$ sind. Insbesondere können die in $X$ vorkommenden $I$-Invarianten höchstens $\Set{1}, \Set{12}, \Set{02}$ sein.

Da für $I=\emptyset, \Set{0}, \Set{2}, \Set{01}, \Set{012}$ bereits $E_I X=0$ gilt, wissen wir $\alpha(E_I X)\subseteq E_I Y$ für diese $I$ erfüllt ist. Aus \ref{matrices:blocks1} folgt dieselbe Inklusion auch für $I=\Set{02}, \Set{12}$. Es bleibt also nur noch $I=\Set{1}$ übrig. Explizites Nachrechnen zeigt, dass $T_0 T_1 T_0$ auf $\operatorname{Eig}_{-v^{-1}}(T_1;X)=E_{\Set{1}} X+E_{\Set{12}} X$ durch Vertauschen von $E_{\Set{1}} X$ und $E_{\Set{12}} X$ operiert. Also folgt:
\[\alpha(E_{\Set{1}} X) = T_0 T_1 T_0 \alpha(E_{\Set{12}} X) \subseteq T_0 T_1 T_0 E_{\Set{12}} Y = E_{\Set{1}} Y\]
Daher ist $\alpha$, wie gewünscht, $\Omega$-linear.
\end{proof} 


\begin{theorem}\label{gyoja:H3}
\index{symbols}{$H_3$,$H_4$}
Gyojas Vermutung ist korrekt für $W=H_3$.
\end{theorem}
\begin{proof}
Es ist eine Liste von $W$-Graphen für jeden Isomorphietyp bekannt, siehe etwa \citep[11.1.8]{geckpfeiffer}. Die eindimensionalen erfüllen $(\Pi_\lambda)$, zweidimensionale gibt es nicht, die dreidimensionalen sind die Spiegelungsdarstellung, ihr Dual sowie die algebraischen Konjugate dieser beiden, erfüllen also auch $(\Pi_\lambda)$.

Übrig bleiben die beiden vier- und die beiden fünfdimensionalen Isomorphietypen. In Tabelle \ref{tab:w_graphs_H3} ist jeweils ein $W$-Graph für diese vier Charaktere angegeben.

\begin{table}[hbp]
\begin{tabular}{lcl}
Name & Grad & $W$-Graph \\
\hline
$4_r$                & 4 & 
	\begin{tikzpicture}
		\node[Vertex] (E_1)  at (0.0,0.0) {$1$};
		\node[Vertex] (E_2)  at (1.5,0.0) {$2$};
		\node[Vertex] (E_13) at (0.0,1.5) {$13$};
		\node[Vertex] (E_23) at (1.5,1.5) {$23$};
		\path[EdgeT]
			(E_1)  edge node[below]{$-1$} (E_2)
			(E_13) edge node[above]{$-1$} (E_23)
			(E_2)  edge node[desc] {$-1$} (E_13);
		\path[EdgeTdir]
			(E_1) edge node[left] {$-1$} (E_13)
			(E_2) edge node[right]{$-1$} (E_23);
	\end{tikzpicture} \\
$4_r'=\sgn\cdot 4_r$ & 4 & 
	\begin{tikzpicture}
		\node[Vertex] (E_1)  at (0.0,0.0) {$1$};
		\node[Vertex] (E_2)  at (1.5,0.0) {$2$};
		\node[Vertex] (E_13) at (0.0,1.5) {$13$};
		\node[Vertex] (E_23) at (1.5,1.5) {$23$};
		\path[EdgeT]
			(E_1)  edge node[below]{$1$} (E_2)
			(E_13) edge node[above]{$1$} (E_23)
			(E_2)  edge node[desc] {$1$} (E_13);
		\path[EdgeTdir]
			(E_1) edge node[left] {$1$} (E_13)
			(E_2) edge node[right]{$1$} (E_23);
	\end{tikzpicture} \\
$5_r$                & 5 & 
	\begin{tikzpicture}
		\node[Vertex] (E_13) at (0.0,0) {$13$};
		\node[Vertex] (E_2a) at (1.5,0) {$2$};
		\node[Vertex] (E_1a) at (3.0,0) {$1$};
		\node[Vertex] (E_2b) at (4.5,0) {$2$};
		\node[Vertex] (E_3)  at (6.0,0) {$3$};
		\path[EdgeT]
			(E_13) edge node[above]{$1$} (E_2a)
			(E_2a) edge node[above]{$1$} (E_1a)
			(E_1a) edge node[above]{$1$} (E_2b)
			(E_2b) edge node[above]{$1$} (E_3);
	\end{tikzpicture} \\
$5_r'=\sgn\cdot 5_r$ & 5 & 
	\begin{tikzpicture}
		\node[Vertex] (E_2)   at (0.0,0) {$2$};
		\node[Vertex] (E_13a) at (1.5,0) {$13$};
		\node[Vertex] (E_23a) at (3.0,0) {$23$};
		\node[Vertex] (E_13b) at (4.5,0) {$13$};
		\node[Vertex] (E_12)  at (6.0,0) {$12$};
		\path[EdgeT]
			(E_2)   edge node[above]{$-1$} (E_13a)
			(E_13a) edge node[above]{$-1$} (E_23a)
			(E_23a) edge node[above]{$-1$} (E_13b)
			(E_13b) edge node[above]{$-1$} (E_12);
	\end{tikzpicture} \\
\end{tabular}
\caption{$W$-Graphen der vier- und fünfdimensionalen Darstellungen von $H_3$}
\label{tab:w_graphs_H3}
\end{table}

Schritt 1: Wir zeigen erst einmal $(\Pi_{5_r})$. Seien dafür $X,Y,\alpha$ wie in der Definition. Die in $X$ vorkommenden $H$-Isomorphietypen können nur noch $4_r, 4_r', 5_r, 5_r'$ sein, da für alle anderen $H$-Isomorphietypen schon $(\Pi^\mu)$ gezeigt wurde. Da in $Y$ nur die Invarianten $\Set{1}, \Set{2}, \Set{3}, \Set{13}$ vorkommen, gilt bereits automatisch $\alpha(E_I X)=0=E_I Y$ für $I=\Set{23},\Set{12},\Set{123}$. Da der triviale Charakter nicht in $X$ vorkommt, gilt auch $E_\emptyset X=0$. Lemma \ref{matrices:blocks1} zeigt außerdem, dass $\alpha(E_I X)\subseteq E_I Y$ für $I=\Set{2}$ gilt. Es bleibt also, die entsprechende Aussage für $I=\Set{1}$ und $I=\Set{3}$ zu zeigen.

Da $T_1$ und $T_3$ kommutieren, bildet $T_3$ den Unterraum $\operatorname{Eig}_{-v^{-1}}(T_1;Z)=E_{\Set{1}} Z + E_{\Set{13}} Z$ in sich selbst ab und umgekehrt, wobei $Z$ von einem der vier Isomorphietypen $4_r, 4_r', 5_r, 5_r'$ sei. Aus den vier $W$-Graphen lesen wir jedoch ab, dass $E_{\Set{1}} = \operatorname{Eig}_{-v^{-1}}(T_1;Z)\cap\operatorname{Eig_v(T_3;Z)}$ bzw. $E_{\Set{3}} = \operatorname{Eig}_{-v^{-1}}(T_3;Z)\cap\operatorname{Eig_v(T_1;Z)}$ gilt. Damit gilt es auch für $Z=X$, da sich diese Gleichung offenbar auf direkte Summen von $H$-Moduln überträgt. Da $\alpha$ diese Eigenräume erhält, gilt nun $\alpha(E_{\Set{s}} X)\subseteq E_{\Set{s}} Y$ für $s=1$ und $s=3$, wie gewünscht.

\bigskip
Wir zeigen als nächstes $(\Pi^{5_r'})$. Seien dafür $X,Y,\beta$ wie in der Definition. Die in $X$ vorkommenden $H$-Isomorphietypen können nur noch $4_r, 4_r', 5_r'$ sein, da für alle anderen $H$-Isomorphietypen schon $(\Pi^\mu)$ gezeigt wurde.  Da in $Y$ nur die Invarianten $\Set{2}, \Set{12}, \Set{13}, \Set{23}$ vorkommen, gilt bereits automatisch $\beta(E_I Y)=0\subseteq E_I X$ für $I=\emptyset,\Set{1},\Set{2},\Set{123}$. Lemma \ref{matrices:blocks1} zeigt außerdem, dass $\beta(E_I Y)\subseteq E_I X$ für $I=\Set{12}, \Set{13}, \Set{23}$ gilt. Es bleibt also, die entsprechende Aussage für $I=\Set{2}$ zu zeigen.

Mit $T_2$ kommutiert nun zwar weder $T_1$ noch $T_3$, aber $h := T_3 T_2 T_1 T_2 T_3$ tut es. Rechnet man explizit nach, so stellt man fest, dass $E_{\Set{2}} Z = h(E_{\Set{12}} Z)$ gilt für $Z$ vom Isomorphietyp $5_r'$.

\end{proof}







\begin{lemma}
Sei $(W,S)$ eine Coxeter-Gruppe vom Typ $A_n$. Sei weiter $k\in\IN$ und $\binom{S}{k}\subseteq 2^S$ die Menge der $k$-elementigen Teilmengen von $S$.

\begin{enumerate}
	\item Definiere $\theta: \binom{S}{k}\to \IZ^k$ durch $\theta(I):=(i_1,i_2,\ldots,i_k)$, wobei $i_1<i_2<\ldots<i_k$ die aufsteigend geordneten Elemente von $I$ seien. $\theta$ ist ein Graphisomorphismus des auf $\binom{S}{k}$ induzierten Untergraphen des Kompatibilitätsgraphen $\mathcal{Q}_W$ auf einen Untergraphen von $\IZ^k$, wobei $x,y\in\IZ^k$ genau dann verbunden seien, wenn ihr euklidischer Abstand $1$ ist. Mit anderen Worten: $\theta(I)$ und $\theta(J)$ sind genau dann durch eine Kante verbunden, wenn $I$ und $J$ es sind.
	\item Es seien $I,J,K,L\in\binom{S}{k}$ die Ecken eines Vierecks in diesem Graphen, d.h. es existieren Kanten $I - J$, $I - K$, $J - L$ und $K - L$. Dann ist dies ein "`kommutatives Quadrat"' in dem Sinne, dass $X_{IJ} X_{JL} = X_{IK} X_{KL}$ in $\OmegaGy$ gilt.
	\item Es seien $I,J\in\binom{S}{k}$ beliebig und $I \leftarrow K_1 \leftarrow K_2 \leftarrow \ldots \leftarrow K_m \leftarrow J$ ein Pfad minimaler Länge von $J$ nach $I$ im Kompatibilitätsgraphen sei, welcher ausschließlich Knoten mit $\abs{K_i}=k$ benutzt. Das Element $Y_{IJ} := X_{I,K_1} X_{K_1,K_2} \cdots X_{K_m, J}$ ist dann von der Wahl dieses Pfades unabhängig.
\end{enumerate}
\end{lemma}
\begin{proof}
a. Sind $I,J\in\binom{S}{k}$ durch eine Kante verbunden, so folgt aus dem obigen Lemma, dass $I\setminus J=\Set{s}$, $J\setminus I=\Set{s\pm 1}$ für genau ein $s\in S$ gilt. O.B.d.A. nehmen wir $J\setminus I=\Set{s+1}$ an. Das heißt, dass $I$ und $J$ die Gestalt $A\dot{\cup}\Set{s}\dot{\cup}B$ bzw. $A\dot{\cup}\Set{s+1}\dot{\cup}B$ für $A,B\subseteq S$ haben, wobei $a<s<s+1<b$ für alle $a\in A, b\in B$ gilt. Daher stimmen $\theta(I)$ und $\theta(J)$ in den ersten $\abs{A}$ und den letzten $\abs{B}$ Koordinaten überein und unterscheiden sich in der restlichen Koordinate genau um den Betrag $1$.

Sind umgekehrt $\theta(I)$ und $\theta(J)$ in allen bis auf einer Koordinate gleich und unterscheiden sich in dieser Koordinate um den Betrag $1$. Dann können wir genau die gleiche Situation herstellen, dass $I=A\dot{\cup}\Set{s}\dot{\cup}B$ und $J=A\dot{\cup}\Set{s+1}\dot{\cup}B$ gilt für $A,B\subseteq S$, die $a<s<s+1<b$ für alle $a\in A, b\in B$ erfüllen. Dann ist $I\setminus J=\Set{s}$ und $J\setminus I=\Set{s+1}$. $s$ und $s+1$ sind im Dynkin-Diagramm verbunden, also sind $I$ und $J$ im Kompatibilitätsgraphen verbunden.

\bigskip
b. Wir nehmen o.B.d.A. an, dass die vier Ecken des Quadrats so bezeichnet sind, dass
\[\begin{array}{rcccl}
	I = A\dot{\cup} & \Set{s}   &\dot{\cup}B\dot{\cup}& \Set{t+1} &\dot{\cup}C \\
	J = A\dot{\cup} & \Set{s}   &\dot{\cup}B\dot{\cup}& \Set{t}   &\dot{\cup}C \\
	K = A\dot{\cup} & \Set{s+1} &\dot{\cup}B\dot{\cup}& \Set{t+1} &\dot{\cup}C \\
	L = A\dot{\cup} & \Set{s+1} &\dot{\cup}B\dot{\cup}& \Set{t}   &\dot{\cup}C
\end{array}\]
für $A,B,C,\subseteq S$ mit $a<s<s+1<b<t<t+1<c$ für alle $a\in A$, $b\in B$ und $c\in C$ gilt.

Das kommutative Quadrat hat dann die in Abbildung \ref{fig:gyoja:comp_graph_comm_square} dargestellt Form und wir müssen zeigen, dass die je zwei verschiedenen Wege von einer Ecke zur gegenüberliegenden Ecke gleich sind. Dazu benutzen wir die Relationen vom Typ $(\gamma)$.
\begin{figure}[ht]
	\input{img/comp_graph_comm_square.tex}
	\caption{Kommutatives Quadrat in $\binom{S}{k}\subseteq\mathcal{Q}_W$}
	\label{fig:gyoja:comp_graph_comm_square}
\end{figure}

Fall 1: $K \leftarrow J$.

Wir benutzen die Relation $(\gamma^{s+1,t+1})$, welche die Form
\[\sum_{U\subseteq S} X_{KU}^{s+1} X_{UJ}^{t+1} = \sum_{V\subseteq S} X_{KV}^{t+1} X_{VJ}^{s+1}\]
hat. Wir beobachten, dass es höchstens ein $U$ mit $\abs{U}=k$ und $X_{KU}^{s+1}\neq 0\neq X_{UJ}^{t+1}$ gibt aufgrund des obigen Lemmas, nämlich $U=I$. Genauso gibt es höchstens ein $V$ mit $\abs{V}=k$ und $X_{KV}^{t+1} \neq 0 \neq X_{VJ}^{s+1}$, nämlich $V=L$. Unser Ziel ist also, dass keine anderen $U$ und $V$ auftreten können.

Angenommen, es gäbe ein $U\subseteq S$ mit $K \xleftarrow{s+1} U \xleftarrow{t+1} J$ und $\abs{U}<k$. Dann ist $U\leftarrow J$ keine Inklusionskante, d.h. aufgrund des obigen Lemmas gilt $\abs{U}=k-1$, $t+2\in J$ und $U=J\setminus\Set{t,t+2}$. Insbesondere muss $t+2\in C$ und $U=A\cup\Set{s}\cup B\cup\Set{t+1}\cup(C\setminus\Set{t+2})$ sein. Daraus folgt $K\setminus U=\Set{s+1,t+2}$ und $U\setminus K=\Set{s}$. Nun gilt jedoch $s+1<t<t+2$, d.h. es gibt keine Kante $s - t+2$ im Dynkin-Diagramm und somit kann es keine Kante $K\leftarrow U$ geben. Das ist der gesuchte Widerspruch.

Angenommen, es gäbe ein $U\subseteq S$ mit $K \xleftarrow{s+1} U \xleftarrow{t+1} J$ und $\abs{U}>k$. Dann ist $K\leftarrow U$ keine Inklusionskante, d.h. aufgrund des obigen Lemmas gilt $\abs{U}=k+1$ und $U=A \dot{\cup} \Set{s,s+2} \dot{\cup} B \dot{\cup} \Set{t+1} \dot{\cup} C$. Es ist insbesondere $s+2\neq t+1$. Wegen $s+1<t$Dann ist jedoch $U\setminus J=\Set{s+2,t+1}$ und $J\setminus U=\Set{t}$. Daraus folgt, dass $s+2=t-1$ sein muss, weil sonst keine Kante $t - s+2$ im Dynkin-Diagramm existieren kann. Insbesondere darf es wegen $s+2<b<t$ keine Elemente in $B$ geben.


\end{proof}

==> ch_cell_alg/block.tex <==
\section{Blocktheorie zellulärer Algebren}

Dieser Abschnitt soll beweisen, dass (modulo harmloser Voraussetzungen) in jeder Zerlegung $A=A_1\times A_2$ einer zellulären Algebra als Produkt zweier Algebren $A_1$ und $A_2$ diese Faktoren ebenfalls zellulär sind. Für bestimmte Koeffizientenringe, etwa Körper, kann man das relativ einfach aus dem schon Bewiesenen (insbesondere \ref{CellAlg:condensation}) ableiten. Dieser Abschnitt hat zum Ziel, diese Aussage im allgemeinen Fall zu beweisen. Dies scheint bisher nicht bekannt gewesen zu sein.

Fixiere also wie zuvor einen kommutativen Ring $R$, eine zelluläre $R$-Algebra $A$ mit Zell-Datum $(\Lambda, M, C, \ast)$.

\subsection{Strukturkonstanten und die invarianten Bilinearformen}

\begin{definition}\label{CellAlg:def:Element_ideals}
Sei $x\in A$ beliebig. Setze dann:
\[\Phi_x:=\bigcap_{\substack{\Phi\subseteq\Lambda\,\text{Ideal} \\ x\in A(\Phi)}} \Phi,\]
\[\Phi_x':=\Set{\lambda\in\Phi | \lambda\,\text{ist nicht maximal in}\,\Phi_x}\quad\text{und}\]
\[\Psi_x := \Phi_x \setminus \Phi_x' = \Set{\lambda | \lambda\,\text{ist maximal in}\,\Phi_x}.\]
\end{definition}

\begin{remark}
\begin{itemize}
	\item Weil $1$ in keinem echten Ideal enthalten ist, ist z.B. $\Phi_1=\Lambda$ und $\Psi_1=$ Menge aller maximalen Elemente von $\Lambda$.
	\item Man beachte auch, dass $\Phi_x=\Phi_{x^\ast}$, weil alle $A(\Phi)$ invariant unter $\ast$ sind.
\end{itemize}
\end{remark}

Das folgende Lemma wird die Vorstellung zementieren, dass eine zelluläre Algebra eine Aufreihung von (verallgemeinerten) Matrizenringen entlang der Ordnung $\Lambda$ ist:
\begin{lemma}[Multiplikation in Termen von $\phi_\lambda$]\label{CellAlg:Multiplication_phi}
Für $\lambda\in\Lambda$ setze $d_\lambda:=\abs{M(\lambda)}$ und $G^\lambda=(g_\mathfrak{st}^\lambda)_{\mathfrak{s},\mathfrak{t}}:=(\phi_\lambda(C_\mathfrak{s},C_\mathfrak{t}))_{\mathfrak{s},\mathfrak{t}} \in R^{d_\lambda\times d_\lambda}$ (d.h. $G^\lambda$ ist die Gram-Matrix von $\phi_\lambda$ bzgl. der kanonischen Basen).

Definiere für $x,y\in A$ und $\lambda\in\Lambda$ die Matrizen $X^\lambda=(x_\mathfrak{st}^\lambda)_{\mathfrak{s},\mathfrak{t}}$, $Y^\lambda=(y_\mathfrak{st}^\lambda)_{\mathfrak{s},\mathfrak{t}}$ und  $Z^\lambda=(z_\mathfrak{st}^\lambda)_{\mathfrak{s},\mathfrak{t}}\in R^{d_\lambda\times d_\lambda}$ durch
	\[x = \sum_{\substack{\lambda\in\Lambda \\ \mathfrak{s},\mathfrak{t}\in M(\lambda)}} x_{\mathfrak{st}}^\lambda C_\mathfrak{st}^\lambda\] 
	\[y = \sum_{\substack{\lambda\in\Lambda \\ \mathfrak{s},\mathfrak{t}\in M(\lambda)}} y_{\mathfrak{st}}^\lambda C_\mathfrak{st}^\lambda\] 
	\[xy = \sum_{\substack{\lambda\in\Lambda \\ \mathfrak{s},\mathfrak{t}\in M(\lambda)}} z_{\mathfrak{st}}^\lambda C_\mathfrak{st}^\lambda\] 

Mit diesen Bezeichnungen gilt:
\begin{enumerate}
	\item Die Matrix von $x^\ast$ ist $(X^\lambda)^T$. Insbesondere ist $x=x^\ast \implies X^\lambda=(X^\lambda)^T$.
	\item Falls $\lambda\in\Psi_x$ ist, so ist $X^\lambda G^\lambda$ die Darstellungsmatrix von $x:W(\lambda)\to W(\lambda)$ und $(X^\lambda)^T G^\lambda$ die Darstellungsmatrix von $x^\ast:W(\lambda)\to W(\lambda)$ (beides bzgl. der kanonischen Basis).
	\item Ist $\lambda\in\Psi_y\cap\Psi_x$, dann ist $X^\lambda G^\lambda Y^\lambda=Z^\lambda$. Ist insbesondere $x$ idempotent, dann gilt $X^\lambda G^\lambda X^\lambda=X^\lambda$ für alle $\lambda\in\Psi_x$.
	\item Ist $x\in Z(A)$ und $\lambda\in\Psi_x$, so ist $X^\lambda G^\lambda = G^\lambda X^\lambda = c1$ für ein geeignetes $c\in R$.
\end{enumerate}
\end{lemma}
\begin{proof}
Die Matrizen $X^\lambda$, bei denen der obere Index $\notin\Phi_x$ ist, sind nach Definition von $\Phi_x$ gleich Null. Wir konzentrieren uns also auf die Indizes aus $\Phi_x$.

\medskip
a. Dafür betrachten wir die Gleichung $x=x^\ast$ modulo $A(\Phi_x')$:
\[x^\ast = \sum_{\lambda} \sum_{\mathfrak{s},\mathfrak{t}\in M(\lambda)} x_\mathfrak{st}^\lambda C_\mathfrak{ts}^\lambda\]
Der Koeffizientenvergleich mit der Definition von $x_\mathfrak{st}^\lambda$ liefert also unmittelbar $x_\mathfrak{st}^\lambda=x_\mathfrak{ts}^\lambda$.

\medskip
b. Es ist $C_\mathfrak{st}^\lambda C_\mathfrak{uv}^\mu \in A(<\lambda)\subseteq A(\Phi_x')$, wenn $\lambda\neq\mu\in \Phi_x$ und $\lambda\in\Psi_x$ ist, denn in diesem Fall ist $\mu$ stets echt kleiner oder unvergleichbar mit $\lambda$. Es sind also nur die Produkte mit gleichem oberen Index interessant. Es ist daher:
\begin{align*}
	x C_\mathfrak{uv}^\lambda &\equiv \sum_{\mathfrak{s},\mathfrak{t}} x_\mathfrak{st} C_\mathfrak{st}^\lambda C_\mathfrak{uv}^\lambda \mod A(<\lambda) \\
	&\equiv \sum_{\mathfrak{s},\mathfrak{t}} x_\mathfrak{st} \phi_\lambda(C_\mathfrak{t},C_\mathfrak{u}) C_\mathfrak{sv}^\lambda \\
	&= \sum_\mathfrak{s} \left(\sum_\mathfrak{t} x_\mathfrak{st} g_\mathfrak{tu} \right) C_\mathfrak{sv}^\lambda \\
	&= \sum_\mathfrak{s} (XG)_\mathfrak{su} C_\mathfrak{sv}^\lambda
\end{align*}
d.h. die Matrix von $x: W(\lambda)\to W(\lambda)$ ist genau $X^\lambda G^\lambda$ wie behauptet. Analog folgt die zweite Aussage.

\medskip
c. Ganz analog können wir $xy$ betrachten:
\[	xy = \sum_{\kappa,\mu} \sum_{\substack{\mathfrak{s},\mathfrak{t}\in M(\kappa) \\ \mathfrak{u},\mathfrak{v}\in M(\mu)}} x_\mathfrak{st}^\kappa y_\mathfrak{uv}^\mu C_\mathfrak{st}^\kappa C_\mathfrak{uv}^\mu \]
Wenn jetzt $\lambda\in\Psi_x\cap\Psi_y$ ist, dann ist auch $\lambda\in\Psi_{xy}$, da $\Phi_{xy}\subseteq\Phi_x\cap\Phi_y$ ist. Die Produkte $C_\mathfrak{st}^\kappa C_\mathfrak{uv}^\mu$ mit $\kappa\in\Phi_x, \mu\in\Phi_y$ haben nur dann Anteile in $\sum RC_\mathfrak{st}^\lambda$, wenn $\kappa=\mu=\lambda$ ist. Wir betrachten also nur obere Indizes gleich $\lambda$:
\begin{align*}
	\sum_{\mathfrak{s},\mathfrak{t},\mathfrak{u},\mathfrak{v}\in M(\lambda)} x_\mathfrak{st}^\lambda y_\mathfrak{uv}^\lambda C_\mathfrak{st}^\lambda C_\mathfrak{uv}^\lambda &\equiv \sum_{\mathfrak{s},\mathfrak{t},\mathfrak{u},\mathfrak{v}} x_\mathfrak{st}^\lambda y_\mathfrak{uv}^\lambda \phi_\lambda(C_\mathfrak{t},C_\mathfrak{u}) C_\mathfrak{sv}^\lambda \mod A(<\lambda) \\
	&= \sum_{\mathfrak{s},\mathfrak{t},\mathfrak{u},\mathfrak{v}} x_\mathfrak{st}^\lambda y_\mathfrak{uv}^\lambda g_\mathfrak{tu}^\lambda C_\mathfrak{sv}^\lambda \\
	&= \sum_{\mathfrak{s},\mathfrak{v}} (X^\lambda G^\lambda Y^\lambda)_\mathfrak{sv} C_\mathfrak{sv}^\lambda
\end{align*}
Vergleichen wir das mit $xy=\sum_\lambda \sum_{\mathfrak{s},\mathfrak{v}} z_\mathfrak{sv}^\lambda C_\mathfrak{sv}^\lambda$, so ergibt sich die Behauptung.

\medskip
d. Diese Aussage bekommen wir dadurch, dass wir $xC_\mathfrak{uv}^\lambda$ mit $C_\mathfrak{uv}^\lambda x$ vergleichen:
\begin{align*}
	x C_\mathfrak{uv}^\lambda &\equiv \sum_{\mathfrak{s},\mathfrak{t}} x_\mathfrak{st}^\lambda C_\mathfrak{st}^\lambda C_\mathfrak{uv}^\lambda \mod A(<\lambda) \\
	&\equiv \sum_{\mathfrak{s},\mathfrak{t}} x_\mathfrak{st}^\lambda \phi_\lambda(C_\mathfrak{t},C_\mathfrak{u}) C_\mathfrak{sv}^\lambda \\
	&= \sum_\mathfrak{s} \left(\sum_\mathfrak{t} x_\mathfrak{st}^\lambda g_\mathfrak{tu}^\lambda \right) C_\mathfrak{sv}^\lambda \\
	&= \sum_\mathfrak{s} (X^\lambda G^\lambda)_\mathfrak{su} C_\mathfrak{sv}^\lambda \\
	C_\mathfrak{uv}^\lambda x &\equiv \sum_{\mathfrak{s},\mathfrak{t}} C_\mathfrak{uv}^\lambda C_\mathfrak{st}^\lambda x_\mathfrak{st}^\lambda  \mod A(<\lambda) \\
	&\equiv \sum_{\mathfrak{s},\mathfrak{t}} C_\mathfrak{ut}^\lambda \phi_\lambda(C_\mathfrak{v},C_\mathfrak{s}) x_\mathfrak{st}^\lambda \\
	&= \sum_\mathfrak{t} C_\mathfrak{ut}^\lambda \left(\sum_\mathfrak{s} g_\mathfrak{vs}^\lambda x_\mathfrak{st}^\lambda \right) \\
	&= \sum_\mathfrak{t} C_\mathfrak{ut}^\lambda (G^\lambda X^\lambda)_\mathfrak{vt} 
\end{align*}
Nur der $C_\mathfrak{uv}^\lambda$-Term kommt in beiden Ausdrücken vor. Wir erhalten also $(X^\lambda G^\lambda)_\mathfrak{su}=0$ für $\mathfrak{s}\neq\mathfrak{u}$, $(G^\lambda X^\lambda)_\mathfrak{vt}=0$ für $\mathfrak{t}\neq\mathfrak{v}$ sowie $(X^\lambda G^\lambda)_\mathfrak{uu} = (G^\lambda X^\lambda)_\mathfrak{vv}$. Da $\mathfrak{u},\mathfrak{v}$ beliebig waren, folgt, dass $X^\lambda G^\lambda = G^\lambda X^\lambda = c1$ ein Vielfaches der Einheitsmatrix ist.
\end{proof}

\begin{remark}
Die Multiplikation $A(\Set{\lambda})\times A(\Set{\lambda})\to A(\Set{\lambda})$ ist also eine verallgemeinerte Matrizenmultiplikation $X \circ_G Y:=XGY$. Die Isomorphieklasse dieses Rings (ggf. ohne Eins) hängt nicht unbedingt von $G$ ab, sondern nur von der Äquivalenzklasse von $A$ unter Multiplikation mit invertierbaren Matrizen, d.h. ist $H=SGT$ mit $S,T\in GL_d(R)$, so ist $(R^{d\times d},\circ_G) \isomorphic (R^{d\times d},\circ_H)$ (siehe auch \ref{CellAlg:example_matrix}).

Falls $R$ ein Hauptidealring ist, kann man beispielsweise nach den Elementarteilern von $G$ schauen. Dies führt u.A. auf die Jantzen-Filtrierung von Zell-Moduln, siehe etwa \cite{mathas1999iwahori}.
\end{remark}

\subsection{Zentrale Idempotente}

\begin{lemma}[Zentrale Idempotente]\label{CellAlg:central_idempotents}
$R$ habe keine nichttrivialen Idempotente.

Sei $e\in A$ ein zentrales Idempotent und $\Phi_e, \Psi_e, X^\lambda, G^\lambda\in R^{d\times d}$ wie in \ref{CellAlg:Multiplication_phi} definiert. Es gilt dann $X^\lambda G^\lambda = 1$ für alle $\lambda\in\Psi_e$. Insbesondere ist also $\det(G^\lambda)\in R^\times$ und $\Psi_e\subseteq\Lambda_\mathfrak{p}^\times$ für alle Primideale $\mathfrak{p}$.
\end{lemma}
\begin{proof}
In \ref{CellAlg:Multiplication_phi} haben wir gezeigt, dass (mit den dortigen Bezeichnungen) $X^\lambda G^\lambda= c1$ für ein $c\in R$ sein muss. Dies ist jedoch die Darstellungsmatrix von $e:W(\lambda)\to W(\lambda)$, also idempotent. $c$ muss also auch idempotent sein. $c$ kann jedoch nicht gleich $0$ sein, sonst wäre $X^\lambda G^\lambda=0$ und somit $X^\lambda=X^\lambda G^\lambda X^\lambda=0$. Es ist aber $\lambda\in\Psi_e$ und daher nach Definition $X^\lambda \neq 0$. Es bleibt daher nur $c=1$ übrig.
\end{proof}

\begin{example}
Auf die Voraussetzungen an $R$ kann nicht verzichtet werden, um $c=1$ zu zeigen. Hat $R$ ein nichttriviales Idempotent $0\neq c\neq 1$, so betrachte die zelluläre Algebra $R^{n\times n}$. Sie hat die beiden Idempotente $cI$ und $(1-c)I$, die wie $c$ bzw. $1-c$ auf $W(\lambda)=R^n$ wirken.
\end{example}

\begin{corollary}
Mit obigen Bezeichnungen und $d_\lambda:=\abs{M(\lambda)}$ ist
\begin{enumerate}
	\item $A/A(\Phi_1') \isomorphic \bigoplus_{\lambda\in\Psi_1} R^{d_\lambda\times d_\lambda}$.
	\item Ist speziell $R$ ein Körper, so gilt zusätzlich $J(A)\subseteq A(\Phi_1')$.
\end{enumerate}
\end{corollary}
\begin{proof}
a. Es sei daran erinnert, dass $\Phi_1=\Lambda$, $\Phi_1'$ ist die Menge der nichtmaximalen Elemente und $\Psi_1$ die Menge der maximalen Elemente von $\Lambda$ ist. Weil die maximalen Elemente paarweise unvergleichbar sind, ist
\[A/A(\Phi_1') = \bigoplus_{\lambda\in\Psi_1} A(\Set{\lambda}) = \bigoplus_{\lambda\in\Psi_1} R^{d_\lambda\times d_\lambda}\]
als $R$-Moduln. Die Identifikation mit den Matrizen ist $C_\mathfrak{st}^\lambda \leftrightarrow E_\mathfrak{st}$. Die Multiplikation zwischen verschiedenen $\lambda$ ist die Nullabbildung.

Der Satz \ref{CellAlg:Multiplication_phi} sagt uns aber, dass in dieser Identifikation die Multiplikation innerhalb des $\lambda$-Anteils durch $(X,Y)\mapsto XG^\lambda Y$ gegeben ist. Obiger Satz sagt aber nun, dass, weil $1$ ein zentrales Idempotent ist, die Matrix $G^\lambda$ invertierbar ist. Die Multiplikation in $R^{d_\lambda\times d_\lambda}$ ist damit zur Matrizenmultiplikation isomorph (siehe das Beispiel  \ref{CellAlg:example_matrix}).

\medskip
b. Ist $R$ ein Körper, so ist $A$ artinsch und daher $J(A)$ charakterisiert als das kleinste Ideal, das einen halbeinfachen Quotienten hat.
\end{proof}

\begin{theorem}[Zerlegungen von zellulären Algebren]
Sei $R$ ein Ring ohne nichttriviale Idempotente.

Betrachte eine Zerlegung $1=\sum_{i=1}^k e_i$ in paarweise orthogonale, zentrale Idempotente. Dann gilt:
\begin{enumerate}
	\item $\Lambda = \bigcup_{i=1}^k \Phi_{e_i}$.
	\item $e_i^\ast = e_i$.
	\item Es gibt für jedes $\lambda\in\Lambda$ genau ein $i\in\Set{1,\ldots,k}$ mit $e_i W(\lambda)=W(\lambda)$. Insbesondere hat jedes $W(\lambda)$ eine Blockzerlegung.
	\item Sind die $e_i$ Blockidempotente, so ist $\Phi_{e_i}$ zusammenhängend, d.h. es gibt keine Zerlegung $\Phi_{e_i} = \Gamma_1\dot{\cup}\Gamma_2$ in nichtleere Teilmengen, sodass alle $\lambda\in\Gamma_1$ mit allen $\mu\in\Gamma_2$ unvergleichbar sind.
\end{enumerate}
\end{theorem}
\begin{proof}
a. Es ist $e_i \in A(\Phi_{e_i})$ nach Definition von $\Phi_{e_i}$. Daher ist $1\in A(\Phi_{e_1})+\ldots+A(\Phi_{e_k})=A(\Phi_{e_1} \cup \ldots\cup \Phi_{e_k})$. Das einzige Ideal von $A$, das $1$ enthält, ist ganz $A=A(\Lambda)$, es muss also $\Lambda = \Phi_{e_1} \cup \ldots\cup \Phi_{e_k}$ sein.

\medskip
b. Sei $e$ ein beliebiges zentrales Idempotent und $\lambda\in\Psi_e$. Dann operiert $e$ als Identität auf $W(\lambda)$ aufgrund von \ref{CellAlg:central_idempotents}. Da $\Phi_e=\Phi_{e^\ast}$ und somit auch $\Psi_e=\Psi_{e^\ast}$ ist, operiert also auch $e^\ast$ als Identität auf $W(\lambda)$. Wir wenden das nun auf die Zerlegung $1=\sum_{i,j} e_i e_j^\ast$ an. Angenommen, es gäbe ein Paar $(i,j)$ mit $i\neq j$ und $e_i e_j^\ast \neq 0$. Dann ist $\Phi_{e_i e_j^\ast}\neq\emptyset$ und wir können ein $\mu\in\Psi_{e_i e_j^\ast}$ wählen. Daraus erhalten wir, dass $e_i e_j^\ast$ und auch $e_j e_i^\ast = (e_i e_j^\ast)^\ast$ als Identität auf $W(\mu)$ operieren. Nun ist aber $e_i e_j^\ast \cdot e_j e_i^\ast = 0$. Das ist ein Widerspruch, also muss $i\neq j \implies e_i e_j^\ast =0$ gelten, d.h. es gilt $e_i = e_i\cdot 1 = \sum_j e_i e_j^\ast = e_i e_i^\ast$. Daher ist $e_i$, wie behauptet, $\ast$-invariant.

\medskip
c. Wir müssen zeigen, dass es ein $i$ mit $\forall j\neq i: e_j W(\lambda)=0$ gibt. Nehmen wir zunächst an, dass $R$ ein Integritätsbereich mit Quotientenkörper $K$ ist. Weil $W(\lambda)\subseteq KW(\lambda)$ ist, reicht es, wenn wir zeigen, dass $e_j KW(\lambda)=0$ ist für alle bis auf ein $j$.

Wir zerlegen zunächst mittels der zentralen Idempotente:
\[KW(\lambda) = \bigoplus_i e_i KW(\lambda)\]
und somit für $KA$-$KA$-Bimoduln:
\[KA(\Set{\lambda}) \isomorphic KW(\lambda)\otimes_K KW(\lambda)^\ast = \bigoplus_{i,j} (e_i KW(\lambda))\otimes(e_j KW(\lambda))^\ast\]
Ist $\alpha: KW(\lambda)\otimes KW(\lambda)^\ast\to KA(\Set{\lambda})$ der Bimodul-Isomorphismus, so ist $\alpha(e_i x\otimes y^\ast e_j^\ast) = e_i \alpha(x\otimes y^\ast)e_j^\ast = e_i e_j \alpha(x\otimes y^\ast)$ für alle $x,y\in W(\lambda)^\ast$ und daher insbesondere $(e_i KW(\lambda))\otimes (e_j KW(\lambda))^\ast=0$ falls $i\neq j$. Wenn wir jetzt $k_i:=\dim_K e_i KW(\lambda)$ setzen, erhalten wir
\[0=\dim_K (e_i KW(\lambda)\otimes KW(\lambda)^\ast e_j^\ast)=(\dim_K e_i KW(\lambda))(\dim_K KW(\lambda)^\ast e_j^\ast)=k_i k_j\]
für alle $i\neq j$. Also ist $k_i\neq 0$ für höchstens ein $i$. Das zeigt die Behauptung für Körper und somit auch für Integritätsringe $R$.

\medskip
Betrachten wir den allgemeinen Fall. Wir erhalten eine Abbildung
\[f: \operatorname{Spec}(R) \to \Set{1,\ldots,k}\]
die jedem Primideal $\mathfrak{p}\in\operatorname{Spec}(R)$ das eindeutig bestimmte $i$ mit $e_i\cdot (R/\mathfrak{p})W(\lambda)\neq 0$ zuordnet. Wir zeigen, dass $f$ stetig bzgl. der Zariski-Topologie auf $\operatorname{Spec}(R)$ und der diskreten Topologie auf $\Set{1,\ldots,k}$ ist.

Sei zunächst $i$ fest, aber beliebig. Betrachte die Menge
\[X_i:=\Set{\mathfrak{p}\in\operatorname{Spec}(R) | e_i\cdot (R/\mathfrak{p})W(\lambda)=0} = f^{-1}(\Set{1,\ldots,k}\setminus\Set{i})\]
Wir zeigen, dass diese Menge abgeschlossen ist. Der Abschluss $\operatorname{cl}(A)$ einer Teilmenge $A\subseteq\operatorname{Spec}(R)$ ist in der Zariski-Topologie durch $V(I(A))$ gegeben, wobei
\[I(A) := \bigcap_{\mathfrak{p}\in A} \mathfrak{p}\]
Es ist $e_i\cdot (R/\mathfrak{p})W(\lambda)=0 \iff e_iW(\lambda) \subseteq \mathfrak{p}W(\lambda)$. Da dies für alle $\mathfrak{p}\in X_i$ gilt, folgt $e_i W(\lambda)\subseteq I(X_i)\cdot W(\lambda)\subseteq\mathfrak{q} W(\lambda)$ für alle $\mathfrak{q}\supseteq I(X_i)$. Also sind alle $\mathfrak{q}$ oberhalb von $I(X_i)$ selbst in $X_i$.

Da nun aber
\[V(I(X_i)) = \Set{\mathfrak{q} | I(X_i)\subseteq\mathfrak{q}}\]
gilt, folgt $\operatorname{cl}(X_i)=V(I(X_i)) \subseteq X_i$, d.h. $X_i$ ist abgeschlossen. Nach Konstruktion von $f$ ist aber $X_i$ das Urbild der abgeschlossenen Menge $\Set{j | j\neq i}$. Mengen dieser Form bilden eine Basis für die abgeschlossenen Mengen der diskreten Topologie. Somit ist $f$ stetig wie behauptet.

Es gilt nun: $\operatorname{Spec}(R)$ ist zusammenhängend genau dann, wenn $R$ keine nichttrivialen Idempotente hat (siehe z.B. \citep[Ex.2.25]{eisenbud}). Das Bild von $\operatorname{Spec}(R)$ unter der stetigen Abbildung $f$ ist zusammenhängend, also einelementig, da $\Set{1,\ldots,k}$ diskret ist. Damit haben wir gezeigt, dass $f$ konstant ist. Es gibt also ein festes $i\in\Set{1,\ldots,k}$, sodass
\[\forall j\neq i\forall\mathfrak{p}\in\operatorname{Spec}(R): e_j W(\lambda)\subseteq \mathfrak{p}W(\lambda)\]
gilt. Der Schnitt über alle Primideale ist das Nil-Radikal $\operatorname{Nil}(R)$ (siehe z.B. \citep[2.12]{eisenbud}), sodass wir $e_j W(\lambda)\subseteq\operatorname{Nil}(R)\cdot W(\lambda)$ erhalten. Die Darstellungsmatrix von $e_j$ hat also nur nilpotente Einträge. Damit ist die Matrix selbst nilpotent. $e_j$ ist aber ein Idempotent, sodass auch die Darstellungsmatrix idempotent sein muss. Das geht nur, wenn es bereits die Nullmatrix ist. Es folgt wie behauptet $\forall j\neq i: e_j W(\lambda) = 0$.

\medskip
d. Gäbe es so eine Zerlegung, wäre $A(\Phi_e) = A(\Gamma_1)\oplus A(\Gamma_2)$ eine Zerlegung in zweiseitige Ideale. Dann wäre aber auch $Ae = A(\Phi_e)e = A(\Gamma_1)e \oplus A(\Gamma_2)e$ eine Zerlegung in zweiseitige Ideale und weil $e$ ein Blockidempotent ist und $Ae$ daher als zweiseitiges Ideal unzerlegbar ist, muss $Ae=A(\Gamma_i)e$ für $i=1$ oder $i=2$ sein. Dann folgt jedoch $Ae\subseteq A(\Gamma_i)$ und somit $\Phi_e\subseteq\Gamma_i$ im Gegensatz zur Annahme $\Gamma_i \subsetneq \Phi$.
\end{proof}

\begin{remark}
Man beachte, dass wir für alle $W(\lambda)$ bewiesen haben, dass es zu genau einem Block gehört, selbst für diejenigen mit $\phi_\lambda=0$. Für $\phi_\lambda\neq 0$ und Integritätsringe $R$ war das schon vorher klar, denn $W(\lambda)$ ist wegen $\Hom_A(W(\lambda),W(\lambda))=R$ (\ref{CellAlg:Hom_cellmodules}) bereits unzerlegbar. Wir haben es jedoch für alle $\lambda\in\Lambda$ und alle zusammenhängenden Ringe $R$ bewiesen, das ist eine stärkere Aussage.
\end{remark}

\begin{corollary}\label{CellAlg:Direkt_factors_are_cellular}
$R$ habe keine nichttrivialen Idempotente und $(A,\ast)$ eine $R$-Algebra mit Involution. Es gilt:
\begin{enumerate}
	\item Ist $A=A_1\oplus A_2$ eine Zerlegung in zweiseitige Ideale, so sind äquivalent:
	\begin{enumerate}
		\item $(A,\ast)$ ist zellulär.
		\item $A_1$ und $A_2$ sind $\ast$-invariant und $(A_1,\ast)$ und $(A_2,\ast)$ sind zellulär.
	\end{enumerate}
	Insbesondere sind also $A_1$ und $A_2$ freie $R$-Moduln und nicht nur einfach projektiv, wenn $A$ zellulär ist.
	\item Sei speziell $A=\bigoplus_{i=1}^k A_i$ eine Blockzerlegung von $A$ (d.h. die $A_i$ seien als zweiseitige Ideale unzerlegbar). In dieser Situation sind äquivalent:
	\begin{enumerate}
		\item $(A,\ast)$ ist zellulär.
		\item Für alle $i$ gilt: $A_i^\ast=A_i$ und $(A_i,\ast)$ ist zellulär.
	\end{enumerate}
	Ggf. kann ein Zelldatum von $A$ gewählt werden, das kompatibel zur Blockzerlegung ist, d.h. $\Lambda = \coprod_i \Lambda^{(i)}$ und $\Set{C_\mathfrak{st}^\lambda | \lambda\in\Lambda^{(i)}}$ ist eine Zell-Basis von $A_i$, und weiterhin die Matrixdarstellungen der Zellmoduln $W(\lambda)$ unverändert lässt.
\end{enumerate}
\end{corollary}
\begin{proof}
b. folgt offenbar induktiv aus a. weshalb es reicht, nur a. zu zeigen.

\medskip
Sind $A_1$ und $A_2$ zellulär, so ist $A$ als direktes Produkt dieser beiden ebenfalls zellulär.

\medskip
Sei also umgekehrt $A$ zellulär und $1=e_1+e_2$ die Zerlegung der Eins als Summe der Einsen von $A_1$ und $A_2$. Weil Nach obigem Satz die zentralen Idempotente $e_i$ invariant unter $\ast$ sind, sind auch die Summanden $A_i = e_i A$ invariant unter $\ast$. Wir konstruieren nun ein Zelldatum für $A_1$ und $A_2$ wie folgt:

Weil laut obigem Satz genau eine der beiden Varianten $e_1 W(\lambda)=W(\lambda)$ bzw. $e_2 W(\lambda)=W(\lambda)$ eintritt, können wir
\[\Lambda^{(i)} := \Set{\lambda\in\Lambda | e_i W(\lambda)=W(\lambda)}\]
definieren. Dann ist $\Lambda=\Lambda^{(1)} \dot{\cup} \Lambda^{(2)}$. Wir setzen außerdem:
\[\forall\lambda\in\Lambda, \mathfrak{s},\mathfrak{t}\in M(\lambda): D_\mathfrak{st}^\lambda := \begin{cases} e_1 C_\mathfrak{st}^\lambda & \lambda\in\Lambda^{(1)} \\ e_2 C_\mathfrak{st}^\lambda & \lambda\in\Lambda^{(2)} \end{cases}\]
Wir behaupten, dass dies eine Zellbasis von $A$ ist.

Weil $e_i$ als Identität auf $W(\lambda)$ operiert für $\lambda\in\Lambda^{(i)}$, operiert es auch als Identität auf $A({\lambda})$. Also gilt:
\[D_\mathfrak{st}^\lambda = e_i C_\mathfrak{st}^\lambda \equiv C_\mathfrak{st}^\lambda \mod A(<\lambda)\]
Daraus ergibt sich, dass die $D$ ein $R$-Erzeugendsystem von $A$ und linear unabhängig sind. Dazu arbeitet man sich jeweils von oben nach unten in der Ordnung und nutzt aus, dass die $C$ bereits eine Basis sind. Das zeigt C1.

Weil $(D_\mathfrak{st}^\lambda)^\ast=(C_\mathfrak{st}^\lambda)^\ast e_i^\ast = e_i C_\mathfrak{ts}^\lambda = D_\mathfrak{ts}^\lambda$ ist, ist auch das Axiom C2 erfüllt. Wieder wegen obiger Gleichung ist auch C3 erfüllt, da das bereits für die C-Basis gilt. Also ist $D$ wie behauptet eine Zell-Basis von $A$. Gewonnen haben wir, dass dies jetzt auch noch eine Zellbasis ist, wenn wir $\Lambda$ durch $\Lambda^{(1)} \coprod \Lambda^{(2)}$ ersetzen, d.h. alle Elemente von $\Lambda_1$ für mit allen Elementen von $\Lambda_2$ unvergleichbar erklären.

Nach Konstruktion ist $\Set{ D_\mathfrak{st}^\lambda | \lambda\in\Lambda^{(i)}, \mathfrak{s},\mathfrak{t}\in M(\lambda)}\subseteq A_i$. Wegen $A=A_1\oplus A_2$ ist diese Menge daher eine $R$-Basis von $A_i$. Das zeigt C1 für $A_i$. C2 und C3 sind erfüllt, weil sie in ganz $A$ gelten.

Weil $e_i$ jeweils als Identität auf $W(\lambda)$ wirkt, folgt auch die Aussage, dass die Zell-Moduln dieser neuen Zell-Basis als Moduln-mit-Basis mit den vorherigen Zell-Moduln übereinstimmen.
\end{proof}

\begin{remark}
\begin{itemize}
	\item Für lokale Integritätsringe kann man die Vererbung der Zellularität auf Blöcke viel einfacher zeigen: Ist $e$ ein Blockidempotent, dann ist $W(\lambda)$ im Block von $e$ für alle $\lambda\in\Psi_e$ wegen \ref{CellAlg:central_idempotents}. Aus $\Psi_e=\Psi_{e^\ast}$ folgt, dass $e=e^\ast$ sein muss. Es ist außerdem $Ae=eAe$. Dann folgt die Behauptung, dass die Blöcke zellulär sind, aus \ref{CellAlg:condensation}. Der eben geführte Beweis ist jedoch deutlich allgemeiner als das.
\end{itemize}
\end{remark}

==> ch_cell_alg/radical.tex <==
\section{Loewy-Länge}

%\textcolor{red}{TODO: Corollary 7.3. in König-Xi \cite{KoenigXi_cellalg_1} gibt $2^n$ als obere Schranke für die Loewy-Länge. Stimmt das??}

\begin{theorem}\label{CellAlg:Nilpotent_ideals_in_cellideals}
Sei $R=K$ ein Körper und $J\subseteq A$ ein Zellideal, $\Delta\subseteq J$, $\alpha: \Delta\otimes_K\Delta^\ast\to J$ wie in der Definition von Zellidealen (\ref{CellAlg:def:Cellideals}). Sei weiter $\phi: \Delta^\ast\otimes_A\Delta\to K$ die assoziierte Bilinearform und $R=\Set{x\in\Delta | \forall y\in\Delta: \phi(y^\ast,x)=0}$ das Radikal von $\phi$.

Definiere dann $I := \alpha(R\otimes\Delta^\ast + \Delta\otimes R^\ast)$. Dann gilt:
\begin{enumerate}
	\item $I$ ist das größte nilpotente Ideal, das in $J$ enthalten ist, d.h. $I=J(A)\cap J$.
	\item Falls $\phi=0$ ist, ist $I=J$ und insbesondere $I^2=0$.
	\item Falls $\phi\neq 0$ aber ausgeartet ist, dann ist $I^3=0\neq I^2$.
	\item Falls $\phi$ nichtausgeartet ist, ist $I=0$.
\end{enumerate}
\end{theorem}
\begin{proof}
Für $\phi=0$ folgt bereits alles aus \ref{CellAlg:def:Cellideals}. Sei also $\phi\neq 0$. Es gilt, wie in \ref{CellAlg:Multiplication_phi} bewiesen, für alle $x,y,z,w\in\Delta$:
\[\alpha(x\otimes y^\ast)\alpha(z\otimes w^\ast) = \phi(y^\ast,z)\alpha(x\otimes w^\ast)\]
Das zeigt, dass $\alpha(R\otimes\Delta^\ast)^2 = \alpha(\Delta\otimes R^\ast)^2 = 0$, $\alpha(\Delta\otimes R^\ast)\alpha(R\otimes\Delta^\ast)=0$ und $\alpha(R\otimes\Delta^\ast)\alpha(\Delta\otimes R^\ast)\subseteq\alpha(R\otimes R^\ast)$ ist. Da $\phi(y^\ast,z)\neq 0$ gewählt werden kann, gilt in der Tat Gleichheit statt der Inklusion, d.h. wir erhalten $I^2=\alpha(R\otimes R)$. Indem wir noch einmal in die obige Gleichung einsetzen, erhalten wir $I^3=0$ wie gewünscht und, falls $R\neq 0$ ist, auch $I^2\neq 0$.

Da $R$ ein $A$-Untermodul von $\Delta$ ist, ist $I$ ein zweiseitiges Ideal. Wir haben also ein nilpotentes Ideal in $J$ gefunden. Es bleibt zu zeigen, dass dies das größte ist. Dazu wählen wir eine Basis $C_\mathfrak{s}$ von $\Delta$, die eine Basis von $R$ enthält. Dann nimmt $\phi$ bzgl. der Basen $C_\mathfrak{s}$ und $C_\mathfrak{s}^\ast$ die Gestalt
\[\begin{pmatrix}	G & 0 \\ 0 & 0 \end{pmatrix}\]
an, wobei $G$ invertierbar ist. $J$ lässt sich mit $K^{d\times d}$ identifizieren und die Multiplikation innerhalb von $J$ ist durch $(X,Y)\mapsto XGY$ gegeben. (siehe \ref{CellAlg:Multiplication_phi}). Das Ideal $I$ ist jetzt gleich der Menge der Matrizen der Form
\[\begin{pmatrix} 0 & \ast \\ \ast & \ast \end{pmatrix}.\]
Es gilt ganz allgemein:
\[\begin{pmatrix} X_{11} & X_{12} \\ X_{21} & X_{22} \end{pmatrix}\cdot_J\begin{pmatrix} Y_{11} & Y_{12} \\ Y_{21} & Y_{22} \end{pmatrix} = \begin{pmatrix} X_{11}GY_{11} & X_{11} G Y_{12} \\ X_{21} G Y_{11} & X_{21} G Y_{12}\end{pmatrix}\]
Da $(X_{11}, Y_{11})\mapsto X_{11} G Y_{11}$ eine Ringstruktur ist, die zum gewöhnlichen Matrizenring isomorph ist (siehe \ref{CellAlg:example_matrix}), kann man aus jedem Element $x\in J\setminus I$ in der oberen, linken Ecke eine beliebige Matrix erzeugen. Daraus kann man dann wiederum in den Positionen $(1,2)$ und $(2,1)$ jede beliebige Matrix erzeugen und daraus wiederum an Position $(2,2)$ jede Matrix. Das heißt, dass das von $x\in J\setminus I$  erzeugte zweiseitige Ideal ist ganz $J$. Da $J^2=J$ ist, kann also $x$ in keinem nilpotenten Ideal enthalten sein.
\end{proof}

\begin{definition}
Setze $\Lambda^{(0)} := \Lambda$ und $\Lambda^{(n+1)} := (\Lambda^{(n)})'=\Set{\lambda\in\Lambda^{(n)}|\lambda\text{ ist nicht max. in }\Lambda^{(n)}}$.
\end{definition}

\begin{theorem}[Loewy-Länge von zellulären Algebren]\label{CellAlg:Loewy_length}
Sei erneut $R=K$ ein Körper. Setze $L:=\min\Set{n\in\IN | \Lambda^{(n)}=\emptyset}$. Dann gilt für die Loewy-Länge  $LL(A):=\min\Set{t\in\IN | J(A)^t=0}$:
\begin{enumerate}
	\item $LL(A)\leq 3^{L-1}$.
	\item $LL(A)\leq 2^n 3^m$, wobei $m:=\#\Set{\lambda\in\Lambda | \phi_\lambda\neq 0 \wedge \rad(\phi_\lambda)\neq 0}$ sei sowie $n:=\#\Set{\lambda\in\Lambda | \phi_\lambda=0}$.
\end{enumerate}
\end{theorem}
\begin{proof}
a. Wir induzieren über $L$. Für $L=1$ sind also alle Elemente von $\Lambda$ maximal, d.h. die sind paarweise unvergleichbar und daher $A$ halbeinfach nach \ref{CellAlg:central_idempotents}. Also ist $J(A)=0$ und $LL(A)=1$ wie behauptet.

Sei nun $L>0$. Dann setzen wir $\Phi:=\Lambda^{(L-1)}$ und betrachten $A/A(\Phi)$. Dies ist eine zelluläre Algebra, auf die wir die Induktionsvoraussetzung anwenden können. Es folgt $J(A)^{3^{L-2}} \subseteq A(\Phi)$ und $A(\Phi)=\bigoplus_{\lambda\in\Phi}  A(\Set{\lambda})$ als $A$-$A$-Bimodul, da alle $\lambda\in\Phi$ minimal in $\Lambda$ sind. Nun ist $I:=J(A)^{3^{L-2}}$ aber ein nilpotentes Ideal und für $\lambda\neq\mu\in\Phi$ gilt $A(\Set{\lambda})A(\Set{\mu})=0$. Also sind sind die Bilder $I_\mu$ von $I$ unter den Projektionen $\pi_\mu: \bigoplus_{\lambda\in\Phi} A(\Set{\lambda}) \to A(\Set{\mu})$ ebenfalls nilpotente Ideale. Insbesondere erhalten wir $I^k\subseteq(\sum_{\mu\in\Phi} I_\mu)^k = \sum_{\mu\in\Phi} I_\mu^k$. Da die $A(\Set{\lambda})$ Zellideale sind ($\lambda\in\Phi$ sind ja minimal), folgt aus obigem Satz also $I^3=0$. Das zeigt die Behauptung in a.

\medskip
b. Die zweite Behauptung folgt nun beinahe genauso. Wir wählen eine topologische Sortierung $\lambda_1\leq \ldots\leq \lambda_k$ von $\Lambda$. Dann hat jede Schicht $\Lambda^{(n)} \setminus \Lambda^{(n+1)}$ genau ein Element. Wir verfolgen dieselbe Induktionsstrategie. Im Induktionsschritt erhalten wir ein nilpotentes Ideal $I$, das im Zellideal $A(\Set{\lambda_1})$ enthalten ist. Je nachdem, welcher der drei Fälle $\phi_{\lambda_1}=0$, $\phi_{\lambda_1}\neq 0$ aber $\rad(\phi_{\lambda_1})\neq 0$ oder eben $\rad(\phi_{\lambda_1})=0$ eintritt, erhalten wir aus obigem Satz $I^2=0$, $I^3=0$ bzw. $I^1=0$. Induktiv folgt dann Aussage b.
\end{proof}

==> ch_wgraphs/matrices.tex <==
\section{Die Blockstruktur in \texorpdfstring{$H$}{H}-linearen Operatoren}

Gyojas Vermutung stellt eine Verbindung zwischen $H$- und $\Omega$-Moduln her. Insbesondere eine der äquivalenten Formulierungen ist interessant: Sind halbeinfache $\Omega$-Moduln, die als Fortsetzungen von isomorphen $H$-Moduln entstehen, bereits als $\Omega$-Moduln isomorph? Oder anders formuliert ist dies eine Frage nach der Rigidität von $W$-Graphen: Wie viel vom $W$"~Gra\-phen wird alleine vom $H$-Modul bestimmt? Dieser Frage wollen wir uns jetzt genauer widmen. 

\begin{lemma}[Rigidität der Eckenlabel]
\index{terms}{Charakter}\index{terms}{Parabolische Untergruppe}
\index{symbols}{$I(x)$}\index{symbols}{$a_\lambda$}
Sei $\omega: KH\to K^{d\times d}$ die Matrixdarstellung eines Geck-$W$-Graphen.
\begin{enumerate}
	\item Für alle reduzierten Darstellungen $w=s_1\ldots s_l$ gilt:
	\[v^{L(w)} \omega(T_w) \in \mathcal{O}^{d\times d} \,\text{und}\, v^{L(w)}\omega(T_w) \equiv \diag(d_x \mid x\in\mathfrak{C})\]
	mit $d_x = (-1)^{l(w)}$ für $\Set{s_1,\ldots,s_l}\subseteq I(x)$ und $d_x=0$ sonst.
	\item Die Multimenge $\mathcal{I}:=\Set{I(x) | x\in\mathfrak{C}}$, d.\,h. die Indexmengen $I(x)$ und die Vielfachheit, mit der sie im $W$-Graph vorkommen, sind eindeutig durch den Charakter von $\omega$ bestimmt.
\end{enumerate}
Ist zusätzlich $\omega$ irreduzibel und vom Isomorphietyp $\lambda\in\Lambda$, dann gilt für die $a$-Invariante die Abschätzung
\begin{enumerate}[resume]
	\item $a_\lambda \geq \max\Set{L(w_{I(x)}) | x\in\mathfrak{C}}$.
	
	Dabei sei $w_J$ das längste Element in der parabolischen Untergruppe $W_J\leq W$ für alle $J\subseteq S$.
\end{enumerate}
\end{lemma}
\begin{proof}
a. Es gilt:
\[v^{L(w)} \omega(T_w) = (v_{s_1} \omega(T_{s_1}))\ldots (v_{s_l}\omega(T_{s_l}))\]
Per definitionem von Geck-$W$-Graphen sind nun die Faktoren $v_s \omega(T_s)\in F[\Gamma_{\geq 0}]$ mit konstantem Term $\diag(s_x)$, wobei
\[s_x=\begin{cases} -1 & s\in I(x) \\ 0 & s\notin I(x)\end{cases}.\]
Daher gilt:
\begin{align*}
	v^{L(w)} \omega(T_w) &\equiv \diag({s_1}_x \mid x\in\mathfrak{C})\cdot \ldots \cdot\diag({s_l}_x \mid x\in\mathfrak{C}) \mod F[\Gamma_{>0}] \\
	&= \diag({s_1}_x \cdot \ldots \cdot {s_l}_x \mid x\in\mathfrak{C})
\end{align*}
Das Produkt $d_x={s_1}_x\cdot\ldots{s_l}_x$ ist genau dann ungleich Null, wenn $s_i\in I(x)$ für alle $i=1\ldots l$ ist. In diesem Fall ist $d_x=(-1)^l=(-1)^{l(w)}$.

\medskip
b. Wir betrachten die Spur von $v^{L(w_J)} \omega(T_{w_J})$ genauer. Wegen der Rechnung in a. ist
\[\tr(v^{L(w_J)}\omega(T_{w_J})) \equiv (-1)^{l(w_J)} \abs{\Set{x\in\mathfrak{C} | J\subseteq I(x)}} \mod\mathfrak{m}.\]
Daher sind die Zahlen $\abs{\Set{x\in\mathfrak{C} | J\subseteq I(x)}}$ für alle $J\subseteq S$ durch den Charakter der Darstellung eindeutig bestimmt. Da
\[\Set{x\in\mathfrak{C} | I(x)=J} = \Set{x\in\mathfrak{C} | J\subseteq I(x)} \setminus \coprod_{J\subsetneq K\subseteq S} \Set{x\in\mathfrak{C} | I(x)=K}\]
gilt, kann man also die Vielfachheiten $\abs{\Set{x\in\mathfrak{C} | I(x)=J}}$ rekursiv berechnen.

\medskip
c. Aus a. folgt, dass für $J\subseteq I(x)$ gilt:
\[v^{L(w_J)}\chi_\lambda(T_{w_J}) = \tr(v^{L(w_J)}\omega(T_{w_J})) \not\equiv 0 \mod \mathfrak{m}\]
Wir haben im Kapitel über balancierte Darstellungen bereits festgestellt, dass für alle $w\in W$ stets $\nu(\chi_\lambda(T_w)) \geq -a_\lambda$ ist. Weil wir nun $\nu(\chi_\lambda(T_{w_J}))=-L(w_J)$ festgestellt haben, muss also $a_\lambda\geq L(w_J)$ sein.
\end{proof}

Zumindest die Teilaussage b. kann man auch für alle $W$-Graphen beweisen, wenn wir ausnutzen, dass $W$-Graph-Moduln nicht nur $H$- sondern auch $\Omega$-Moduln sind:
\begin{lemma}\label{matrices:unique_I_inv}
\index{symbols}{$I(x)$}
Sei $V$ ein $\Omega$-Modul. Dann gilt:
\[e_s V = \Set{x\in V | e_s x=-v_s^{-1} x} = \operatorname{Eig}_{-v_s^{-1}}(T_s;V)\]
Ist speziell $V$ der $W$-Graph-Modul des $W$-Graphen $(\mathfrak{C},I,m)$, so sind die Vielfachheiten der Eckenlabel, d.\,h. die Dimensionen $\dim_K E_I V$, eindeutig durch den $H$"~Isomorphietyp von $V$ bestimmt.
\end{lemma}
\begin{proof}
Ist $u\in e_s V$, dann ist:
\begin{align*}
	\iota(T_s) u &= (-v_s^{-1} e_s+v_s (1-e_s)+x_s)(e_s u) \\
	&= (-v_s^{-1} \underbrace{e_s^2}_{=e_s}+v_s \underbrace{(1-e_s)e_s}_{=0}+\underbrace{x_s e_s}_{=0}) u \\
	&= -v_s^{-1} e_s u \\
	&= -v_s^{-1} u \\
	\implies u&\in\operatorname{Eig}_{-v_s^{-1}}(T_s;V)
\end{align*}
Und andersherum: Wenn $T_s u = -v_s^{-1} u$ gilt, folgt:
\begin{align*}
	-v_s^{-1} e_s u + v_s(1-e_s)u + x_s u &= -v_s^{-1} u \\
	\implies v_s (1-e_s) u + x_s u &= -v_s^{-1}(1-e_s) u \\
	\implies v_s \underbrace{(1-e_s)^2}_{=1-e_s} u + \underbrace{(1-e_s) x_s}_{=0} u &= -v_s^{-1}(1-e_s)^2u \\
	\implies v_s(1-e_s) u &= -v_s^{-1}(1-e_s)u \\
	\implies (1-e_s) u &= 0 \\
	\implies u &\in e_s V
\end{align*}
Aus $e_s = \sum_{s\in I} E_I$ folgt, dass $\bigcap_{s\in I} e_s V = \bigoplus_{J\supseteq I} E_J V$ sich eindeutig durch die Operation der $T_s$ charakterisieren lässt. Wir erhalten insbesondere, dass die Vielfachheit von $I$
\[\abs{\Set{x\in\mathfrak{C} | I(x)=I}} = \dim E_I V = \dim \frac{\bigcap_{s\in I} \operatorname{Eig}_{-v_s^{-1}}(T_s; V) }{ \sum_{s\notin I} \bigcap_{t\in I\cup\Set{s}} \operatorname{Eig}_{-v_t^{-1}}(T_t;V) }\]
eindeutig durch die $H$-Operation auf $V$ bestimmt ist.
\end{proof}

\begin{remark}
\begin{itemize}
	\item Im endlichdimensionalen Fall können wir die Vielfachheiten in der Tat alleine aus dem Charakter $\chi_V$ von $V$ bestimmen: Wenn wir $V=\bigoplus_{\chi\in\Irr(H)} V_\chi$ für die Zerlegung in homogene Komponenten schreiben, ist die Signumskomponente genau $V_{\textrm{sgn}}=\bigcap_{s\in S} \operatorname{Eig}_{-v_s^{-1}}(T_s;V)$. Allgemeiner ist $\bigcap_{s\in I} \operatorname{Eig}_{-v_s^{-1}}(T_s;V)$ genau die Signumskomponente von $\text{Res}_{H_I}^H (V)$. Die Dimensionen sind also genau gleich den Vielfachheiten des Signumscharakters in $\chi_V$.
	\item In der Tat können wir diese Vielfachheiten schon aus dem Charakter des $F[W]$"~Mo\-duls bestimmen, welcher entsteht, wenn wir $V$ mit $v^\gamma\mapsto 1$ spezialisieren. Es kann also ausschließlich mit der Coxeter-Gruppe gerechnet werden, es ist keine Rechnung in $H$ nötig.
\end{itemize}
\index{term}{Signum}\index{terms}{Charakter}
\end{remark}

\begin{convention}
Bis auf die Anordnung der Zeilen und Spalten legt der $H$-Isomorphietyp von $\omega$ also fest, welche Indizes $x$ welches $I(x)$ haben. Das legt nahe, die Zeilen und Spalten von $m^s$, $\omega(T_s)$ etc. von vornherein so zu sortieren, dass Indizes mit identischen Eckenlabeln gruppiert werden. Wir vereinbaren, dass ab jetzt für alle im Zusammenhang mit $W$-Graphdarstellungen vorkommenden Matrizen stets diese Blockstruktur verwendet wird. Die Blöcke sind also durch $2^S$ indiziert (wobei leere Blöcke vorkommen dürfen). Wir bezeichnen die Teilblöcke jeder Matrix $A$ entsprechend mit $A_{IJ}$.
\end{convention}

\begin{lemma}[$H$-Homomorphismen sind Blockdreiecksmatrizen]\label{matrices:blocks1}
\index{terms}{Blockmatrix}\index{terms}{Blockmatrix!Blockdreiecksmatrix}
Seien $V, W$ beliebige $K\Omega$-Moduln. Ist $\alpha\in\Hom_H(V,W)$, dann gilt
\[\alpha(E_I V) \subseteq \sum_{J\supseteq I} E_J W\]
Wenn wir je eine den Zerlegungen $V=\bigoplus_{I\subseteq S} E_I V$ bzw. $W=\bigoplus_{I\subseteq S} E_I W$ angepasste Basis wählen, heißt das, dass die Matrix $A$ von $\alpha$ eine Blockdreiecksmatrix bzgl. der Inklusion ist.
\end{lemma}
\begin{proof}
Es gilt $e_s V = \operatorname{Eig}_{-v_s^{-1}}(T_s;V)$ wie oben gesehen. Da $\alpha$ $H$-linear ist, bildet es Eigenräume ineinander ab, d.\,h. es gilt $\alpha(\operatorname{Eig}_{-v_s^{-1}}(T_s;V)) \subseteq \operatorname{Eig}_{-v_s^{-1}}(T_s;W)$. Es gilt somit $\alpha(e_s V)\subseteq e_s W$. Wegen $e_s = \bigoplus_{s\in I} E_I$ ist $\bigcap_{s\in I} e_s V = \sum_{I\subseteq J} E_I V$ und daraus folgt $\alpha(\sum_{J\subseteq I} E_I V) \subseteq \sum_{J\subseteq I} E_J W$.
\end{proof}

\begin{remark}
\index{terms}{Blockmatrix!Blockdiagonalmatrix}
Eine der äquivalenten Varianten von Gyojas Vermutung ist, dass für halbeinfache $V,W$ solch ein $\alpha$ automatisch $\Omega$-linear sein sollte, d.\,h. $\alpha(E_I V)\subseteq E_I W$ für alle $I\subseteq S$. Mit anderen Worten: Die Darstellungsmatrix von $\alpha$ sollte nicht nur eine Blockdreiecks-, sondern eine Blockdiagonalmatrix sein.
\end{remark}

Speziell für endlichdimensionale Räume können wir ein bisschen mehr über die Blockstruktur von $H$-linearen Operatoren aussagen:
\begin{lemma}[Blockstruktur]\label{matrices:off_diagonal}
\index{terms}{Blockmatrix}
Seien $\omega_1, \omega_2: KH\to K^{d_i\times d_i}$ Geck-$W$-Graphendarstellungen, die $GL_d(K)$-äquivalent sind. Insbesondere haben sie also dieselben Eckenlabel in derselben Vielfachheit.
\begin{enumerate}
	\item Ist $A\in\mathcal{O}^{d_2\times d_1}$ mit $A\omega_1 = \omega_2 A$, dann ist automatisch $A_{IJ}\equiv 0\mod\mathfrak{m}$ für alle $I\neq J\in\mathcal{I}$. Mit anderen Worten: Die Reduktion $A\mod\mathfrak{m}$ ist eine Blockdiagonalmatrix.
	\item Ist $B\in\mathcal{O}^{d_1\times d_1}$ eine invariante Bilinearform für $\omega_1$, d.\,h. $\forall h\in H: B\omega_1(h) = \omega_1(h^\ast)^T B$, dann ist automatisch $B_{IJ}\equiv 0\mod\mathfrak{m}$ für alle $I\neq J\in\mathcal{I}$. Mit anderen Worten: Die Reduktion $B\mod\mathfrak{m}$ ist eine Blockdiagonalmatrix.
\end{enumerate}
\end{lemma}
\begin{proof}
Wir beweisen beide Aussagen gemeinsam. Dafür setzen wir der einfacheren Schreibweise wegen $\omega_1:=\omega$ und $\omega_2(T_s):=\omega(T_s)^\text{Tr}$, $A:=B$ in der Situation von b.

Sei zunächst $s\in S$ fest. Wir organisieren die Blöcke so, dass die $I$ mit $s\in I$ zuerst stehen und dann die mit $s\notin I$. Dann gilt $v_s\omega_i(T_s)\in\mathcal{O}^{d\times d}$ und
\[v_s\omega_i(T_s) = \begin{pmatrix} -1 & v_s m^s \\ 0 & v^2 \end{pmatrix} \equiv \begin{pmatrix}	-1 & 0 \\	0 & 0\end{pmatrix}\mod\mathfrak{m}\]
nach Definition von Geck-$W$-Graphen.

Es folgt:
\begin{align*}
	A\cdot v_s\omega_1(T_s) &\equiv \begin{pmatrix}
	A_{11} & A_{12} \\ A_{21} & A_{22}
	\end{pmatrix}\cdot\begin{pmatrix}
	-1 & 0 \\ 0 & 0
	\end{pmatrix} \\
	&=\begin{pmatrix}
	-A_{11} & 0 \\
	-A_{21} & 0
	\end{pmatrix} \\
	v_s\omega_2(T_s)\cdot A &\equiv \begin{pmatrix}
	-1 & 0 \\ 0 & 0
	\end{pmatrix}\cdot\begin{pmatrix}
	A_{11} & A_{12} \\ A_{21} & A_{22}
	\end{pmatrix} \\
	&=\begin{pmatrix}
	-A_{11} & -A_{12} \\ 0 & 0
	\end{pmatrix}
\end{align*}
Es folgt also $A_{12}\equiv 0\mod\mathfrak{m}$ und $A_{21}\equiv 0\mod\mathfrak{m}$. In Indizes geschrieben:
\[\forall x,y: (s\in I(x)\setminus I(y)) \implies A_{xy} \equiv A_{yx} \equiv 0 \mod\mathfrak{m}.\]
Ist jetzt $I(x)\neq I(y)$, dann gibt es immer ein $s\in I(x)\setminus I(y)$ oder ein $s\in I(y)\setminus I(x)$, d.\,h. wir können diese Überlegungen für dieses $s$ anwenden und erhalten $A_{xy}\equiv A_{yx} \equiv 0$. Das zeigt die Behauptungen.
\end{proof}

\begin{remark}
\begin{itemize}
	\item Dieses Lemma beantwortet die Frage von Jürgen Müller (\cite{mueller2012strictlybalanced}), ob Geck-$W$-Graphen, wenn sie balanciert sind (siehe Vermutung \ref{conj:geck_mueller}), bereits automatisch strikt balanciert im Sinne von \ref{balanced_reps:strictly_balanced} seien.

	Zum einen sagt das Lemma, dass dies zutrifft, falls die im $W$-Graph vorkommenden Index-Mengen $I(x)$ höchstens mit Vielfachheit Eins vorkommen. Dann sind die Blöcke nämlich $1\times 1$ und $B\mod\mathfrak{m}$ ist eine Diagonalmatrix.
	
	Ist jedoch die Vielfachheit einer Index-Menge echt größer $1$, dann gibt es einen $l\times l$-Block $B_{II}$ in $B$ mit $l>1$. Nun können wir in diesem Block mit einer beliebigen $l\times l$-Matrix $Q_{II}\in GL_l(F)$ konjugieren und erhielten die Matrix $Q^T B_{II} Q$ im entsprechenden Block der neuen invarianten Bilinearform. Selbst, wenn also $B_{II}\mod\mathfrak{m}$ diagonal wäre, die neue Matrix wäre es im Normalfall nicht mehr. Füllen wir die restlichen Blöcke $Q_{JJ}$ mit der Einheitsmatrix, erhalten wir eine Blockdiagonalmatrix $Q\in GL_d(F)$, d.\,h. die Darstellungsmatrix einer $\Omega$-linearen Abbildung. Wir erhielten nach Basiswechsel mit $Q$ also erneut eine balancierte $W$-Graph-Darstellung, die nun jedoch nicht mehr strikt balanciert ist.
	\index{terms}{Darstellung!balancierte!strikt}

	\item Dasselbe Argument funktioniert aber auch umgekehrt: Wenn $\rho$ balanciert, aber noch nicht strikt balanciert ist, können wir in jedem Diagonalblock von $B$ eine Cholesky-Zerlegung $B_{II}\mod\mathfrak{m} = L_I D_I L_I^T$ durchführen (d.\,h. $L_I$ ist eine untere Dreiecksmatrix mit Einsen auf der Diagonalen, und $D_I$ ist eine Diagonalmatrix) und erhalten eine Blockdreiecksmatrix $L\in GL_d(F)$ derart, dass $L^{-1}\rho L$ eine strikt balancierte $W$-Graph-Darstellung ist.
	\index{terms}{Cholesky-Zerlegung}
\end{itemize}
\end{remark}

\begin{corollary}[Geck-$W$-Graphen als $\Omega$-Moduln]\label{matrices:iota_shriek}
\index{terms}{W-Graph@$W$-Graph!Geck-}
\index{symbols}{\textbf{Mod}}\index{symbols}{\textbf{ssMod}}\index{symbols}{$\iota^\ast$}\index{symbols}{$\iota_"!$}
Es gilt:
\begin{enumerate}
	\item Sind $\omega_1, \omega_2: KH\to K^{d\times d}$ zwei Geck-$W$-Graphen, dann gilt: Sind sie $GL_d(F)$"~kon\-ju\-giert, dann sind sie bereits als $\Omega$-Moduln isomorph.
	\item Sei $KH-\textbf{Mod}$ die volle Modulkategorie und $K\Omega-\textbf{ssMod}$ die Kategorie der halbeinfachen $K\Omega$-Moduln. Es gibt einen Funktor $\iota_!: KH-\textbf{Mod}\to K\Omega-\textbf{ssMod}$ derart, dass $\iota^\ast\circ\iota_!\homotopic\id$, d.\,h. die Fortsetzung von $KH$-Moduln zu $K\Omega$-Moduln via $W$-Graphen kann funktoriell erfolgen.
\end{enumerate}
\end{corollary}
\begin{proof}
a. Ist $A\in GL_d(F)$ mit $A\omega_1 = \omega_2 A$, dann sagt uns das Lemma, dass $A$ (was mit $A\mod\mathfrak{m}$ übereinstimmt) eine Blockmatrix ist, d.\,h. $A\in GL_\mathcal{I}(F)\subseteq\Hom_\Omega(\omega_1,\omega_2)$. Also sind $\omega_1$, $\omega_2$ als $\Omega$-Moduln isomorph.

\bigskip
b. Nun zum Funktor. Auf Objekten ist klar, wie das funktionieren muss: Wir wählen für jeden Isomorphietyp $\lambda\in\Lambda$ einen $W$-Graph-Modul $\omega_\lambda: KH\to K^{d_\lambda\times d_\lambda}$ mit $\omega_\lambda = \overline{\omega_\lambda}\circ\phi$ (deren Existenz ja durch \ref{lusztig_hom:ex_of_w_graphs} gesichert ist). $\iota_!(\omega_\lambda)$ soll dann die Fortsetzung von $\omega_\lambda$ auf $\Omega$ sein. $KH-\textbf{Mod}$ ist halbeinfach, d.\,h. wir können weiter $\iota_!(\bigoplus_{i\in I} \omega_{\lambda_i}) := \bigoplus_{i\in I} \iota_!(\omega_{\lambda_i})$ setzen und haben jedem Isomorphietyp von Objekten ein Bild zugeordnet.

Aus a. folgt nun, dass jeder $H$-Homomorphismus $\omega_\lambda\to\omega_\mu$ bereits $K\Omega$-linear ist, denn Null ist sicherlich $\Omega$-linear und jedes $A\in GL_d(K)$ mit $A\omega_1=\omega_2 A$ ist aufgrund von Lemma \ref{h_vs_j:conj_class} und Schurs Lemma von der Form $k A'$ mit $A'\in GL_d(F), k\in K^\times$. Nun ist $k\id$ sicherlich $\Omega$-linear. Aus a. folgt, dass $A'$ ein $\Omega$-Isomorphismus ist. Daher ist jeder $H$-Homomorphismus $\bigoplus_{i\in I} \omega_{\lambda_i} \to \bigoplus_{j\in J} \omega_{\mu_j}$ in der Tat schon $\Omega$-linear und wir können $\iota_!(f)=f$ für Homomorphismen definieren. Es ist klar, dass dies ein Funktor auf dem Skelett $\Set{\bigoplus_{i\in I} \omega_{\lambda_i}}\subseteq KH-\textbf{Mod}$ ist und $\iota^\ast\circ\iota_!=\id$ wird nach Konstruktion erfüllt. Indem wir jetzt noch eine Äquivalenz von $KH-\textbf{Mod}$ auf dieses Skelett dazuschalten, erhalten wir die Aussage.
\end{proof}

\begin{corollary}[Kategorielle Formulierung von Gyojas Vermutung]
\index{terms}{Vermutung von!Gyoja!Kategorielle Formulierung}
Mit den Bezeichnungen aus dem eben bewiesenen Lemma sind äquivalent:
\begin{enumerate}
	\item Gyojas Vermutung.
	\item $\iota^\ast$ ist voll.
	\item $\iota^\ast$ ist eine Äquivalenz.
	\item $\iota_!$ ist essentiell surjektiv, d.\,h. jede Isomorphieklasse von $K\Omega$-Moduln wird getroffen.
	\item $\iota_!$ ist eine Äquivalenz.
	\item $\iota_!$ ist rechts- oder linksadjungiert zu $\iota^\ast$.
\end{enumerate}
\end{corollary}
\begin{proof}
Wegen $\iota^\ast\circ\iota_! \homotopic \id$ ist $\iota^\ast$ essentiell surjektiv. Treu ist $\iota^\ast$ sowieso, weil es ja der Einschränkungsfunktor ist, also auf Morphismenmengen als Identität wirkt. Zu einer Äquivalenz fehlt also nur, dass $\iota^\ast$ voll ist (siehe z.\,B. \cite{maclane}). Das zeigt b.$\iff$c. Weil "`voll"' hier bedeutet, dass jede $H$-lineare Abbildung zwischen halbeinfachen $\Omega$-Moduln bereits $\Omega$-linear ist, gilt auch a.$\iff$b.

Da $\iota^\ast$ linksinvers zu $\iota_!$ ist, gilt c.$\iff$e. Ein analoges Argument wie zuvor zeigt d.$\iff$e.: $\iota_!$ ist treu wegen $\iota^\ast\circ\iota_!\homotopic\id$ und nach Konstruktion voll. Zu einer Äquivalenz fehlt also nur, dass $\iota_!$ essentiell surjektiv ist.

Zueinander inverse Äquivalenzen sind immer auch zueinander rechts- und linksadjungiert (siehe erneut \cite{maclane}). Daher ist c.$\implies$f. automatisch wahr. Sei für die Umkehrung $\Hom_H(X,\iota^\ast Y) \isomorphic \Hom_\Omega(\iota_! X,Y)$ für alle $X\in KH-\textbf{Mod}$ und alle ${Y\in K\Omega-\textbf{ssMod}}$. Setzen wir für $Y$ einen beliebigen einfachen $K\Omega$-Modul und für $X$ einen einfachen $KH$"~Un\-ter\-mo\-dul ein, so ist $\Hom_H(X,\iota^\ast Y)\neq 0$, d.\,h. es gibt einen von Null verschiedenen $\Omega$-Homomorphismus $\iota_! X\to Y$. Weil $\iota_!X$ und $Y$ einfach sind, muss also $\iota_! X\isomorphic Y$ sein. Analog folgt auch aus $\Hom_\Omega(Y,\iota_! X) \isomorphic \Hom_H(\iota^\ast Y,X)$, dass alle einfachen $K\Omega$-Moduln bereits von einfachen $KH$-Moduln herkommen. Das zeigt f.$\implies$d.
\end{proof}

==> lebenslauf.tex <==
\addchap{Lebenslauf}

\begin{tabular}{p{3cm}p{11cm}}
\textbf{Zur Person} & \\
\hline
Name & Hahn \\
Vorname & Johannes \\
Geburtsdatum & 20.01.1987 \\
Geburtsort & Rostock
\vspace{1em} \\

\textbf{Schulbildung} & \\
\hline
09/1993-08/1997	& Grundschule Rostock Toitenwinkel \\
09/1997-06/2005	& Käthe-Kollwitz-Gynmasium Rostock, Abitur mit Gesamtnote 1,6
\vspace{1em} \\

\textbf{Studium} & \\
\hline
09/2005-03/2006	& Mathematikstudium mit Nebenfach Informatik an der Fernuniversität Hagen \\
04/2006-06/2010	& Mathematikstudium mit Nebenfach Informatik an der Universität Rostock, Diplom mit Gesamtnote 1,1 (Thema "`Van Kampen diagrams and Tarski monster groups"', Betreuer Prof.\,Dr.\, Reinhard Knörr)
\vspace{1em} \\

\textbf{Berufslaufbahn} \\
\hline
seit 08/2010 & Wissenschaftlicher Mitarbeiter der Universität Jena
\end{tabular}

\vspace{2cm}
\underline{\textbf{Vorträge}}

\begin{itemize}
	\item 27.04.2010 "`Van-Kampen-Diagramme und Tarski-Monster-Gruppen"'
	
	Oberseminar der AG Algebra Jena 

	\item 11.05.2012 "`$W$-Graphdarstellungen"'
	
	Fachgruppen-Tagung 2012 der Fachgruppe Computeralgebra, Kassel

	\item 24.11.2012 "`Conjectures about Gyoja's $W$-graph algebra"'
	
	Darstellungstheorietage 2012, Magdeburg

	\item 05.11.2013 "`Structural properties of $W$-graphs"'
	
	Algebra-Seminar Halle-Jena WS 2013/14, Jena
\end{itemize}

\vspace{2cm}
\underline{\textbf{Publikationen}}

\begin{itemize}
	\item Mitautor von "`Mathematisch für Anfänger"', Spektrum Akademischer Verlag, 2009, ISBN 987-3827422859

	\item Mitautor von "`Mathematisch für fortgeschrittene Anfänger"', Spektrum Akademischer Verlag, 2010, ISBN 987-3827426062
\end{itemize}

